Evaluating language models as risk scores

Current question-answering benchmarks predominantly focus on accuracy in realizable prediction tasks. Conditioned on a question and answer-key, does the most likely token match the ground truth? Such benchmarks necessarily fail to evaluate LLMs' ability to quantify ground-truth outcome uncertainty. In this work, we focus on the use of LLMs as risk scores for unrealizable prediction tasks. We introduce folktexts, a software package to systematically generate risk scores using LLMs, and evaluate them against US Census data products. A flexible API enables the use of different prompting schemes, local or web-hosted models, and diverse census columns that can be used to compose custom prediction tasks. We evaluate 17 recent LLMs across five proposed benchmark tasks. We find that zero-shot risk scores produced by multiple-choice question-answering have high predictive signal but are widely miscalibrated. Base models consistently overestimate outcome uncertainty, while instruction-tuned models underestimate uncertainty and produce over-confident risk scores. In fact, instruction-tuning polarizes answer distribution regardless of true underlying data uncertainty. This reveals a general inability of instruction-tuned LLMs to express data uncertainty using multiple-choice answers. A separate experiment using verbalized chat-style risk queries yields substantially improved calibration across instruction-tuned models. These differences in ability to quantify data uncertainty cannot be revealed in realizable settings, and highlight a blind-spot in the current evaluation ecosystem that folktexts covers.

==> tables/both_prompting_schemes_different_rows/acsemployment.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\shortstack{Prompting\\ scheme}}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{ROC \\ AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
\multirow{2}{*}{GPT 4o mini (it)} & Num. & 0.23 & 0.23 & 0.80 & 0.73 & \cellcolor{cyan!0.3} 0.77 & 0.28 \\
 & Q\&A & 0.28 & 0.29 & 0.79 & 0.65 & 0.74 & 0.41 \\
\multirow{2}{*}{Llama 3 70B (it)} & Num. & \cellcolor{cyan!2.6} 0.05 & \cellcolor{cyan!25.0} 0.14 & \cellcolor{cyan!25.0} 0.88 & \cellcolor{cyan!25.0} 0.81 & \cellcolor{cyan!25.0} 0.81 & 0.32 \\
 & Q\&A & 0.17 & 0.19 & \cellcolor{cyan!13.5} 0.85 & 0.73 & \cellcolor{cyan!8.0} 0.78 & 0.29 \\
\multirow{2}{*}{Llama 3 70B} & Num. & \cellcolor{cyan!1.9} 0.05 & \cellcolor{cyan!17.5} 0.15 & \cellcolor{cyan!14.6} 0.86 & \cellcolor{cyan!5.9} 0.78 & \cellcolor{cyan!4.2} 0.78 & 0.31 \\
 & Q\&A & 0.25 & 0.26 & 0.82 & 0.52 & 0.74 & 0.12 \\
\multirow{2}{*}{Llama 3 8B (it)} & Num. & 0.08 & \cellcolor{cyan!0.7} 0.17 & 0.82 & 0.77 & 0.77 & 0.29 \\
 & Q\&A & 0.07 & 0.19 & 0.79 & 0.74 & 0.74 & 0.22 \\
\multirow{2}{*}{Llama 3 8B} & Num. & 0.15 & 0.23 & 0.75 & \cellcolor{orange!23.6} 0.46 & 0.68 & 0.11 \\
 & Q\&A & 0.34 & 0.34 & 0.76 & \cellcolor{orange!25.0} 0.45 & 0.69 & 0.06 \\
\multirow{2}{*}{Mixtral 8x22B (it)} & Num. & 0.06 & \cellcolor{cyan!22.2} 0.14 & \cellcolor{cyan!24.5} 0.87 & \cellcolor{cyan!16.5} 0.79 & \cellcolor{cyan!21.1} 0.80 & 0.33 \\
 & Q\&A & \cellcolor{orange!23.0} 0.38 & \cellcolor{orange!11.0} 0.39 & 0.60 & 0.51 & 0.60 & 0.26 \\
\multirow{2}{*}{Mistral 8x22B} & Num. & 0.15 & 0.18 & 0.82 & \cellcolor{cyan!20.8} 0.80 & \cellcolor{cyan!15.7} 0.79 & 0.35 \\
 & Q\&A & 0.21 & 0.24 & \cellcolor{cyan!15.2} 0.86 & 0.52 & \cellcolor{cyan!3.4} 0.78 & 0.08 \\
\multirow{2}{*}{Mixtral 8x7B (it)} & Num. & 0.07 & \cellcolor{cyan!17.5} 0.15 & \cellcolor{cyan!23.4} 0.87 & \cellcolor{cyan!7.3} 0.78 & \cellcolor{cyan!8.0} 0.78 & 0.27 \\
 & Q\&A & 0.22 & 0.24 & 0.82 & 0.73 & 0.75 & 0.44 \\
\multirow{2}{*}{Mistral 8x7B} & Num. & 0.08 & 0.17 & 0.81 & 0.73 & 0.75 & 0.25 \\
 & Q\&A & 0.30 & 0.31 & 0.81 & \cellcolor{orange!24.3} 0.45 & 0.74 & 0.06 \\
\multirow{2}{*}{Mistral 7B (it)} & Num. & \cellcolor{cyan!8.7} 0.04 & 0.19 & 0.79 & 0.69 & 0.76 & 0.27 \\
 & Q\&A & \cellcolor{orange!6.7} 0.35 & 0.36 & 0.72 & 0.63 & 0.66 & 0.49 \\
\multirow{2}{*}{Mistral 7B} & Num. & 0.14 & 0.19 & 0.80 & \cellcolor{cyan!13.0} 0.79 & \cellcolor{cyan!11.9} 0.79 & 0.42 \\
 & Q\&A & 0.26 & 0.30 & 0.76 & \cellcolor{orange!25.0} 0.45 & 0.69 & 0.04 \\
\multirow{2}{*}{Yi 34B (it)} & Num. & 0.15 & 0.21 & 0.81 & 0.51 & \cellcolor{cyan!13.4} 0.79 & 0.18 \\
 & Q\&A & 0.14 & 0.21 & 0.79 & 0.69 & 0.73 & 0.20 \\
\multirow{2}{*}{Yi 34B} & Num. & 0.13 & 0.23 & 0.66 & 0.50 & 0.64 & 0.11 \\
 & Q\&A & 0.08 & 0.23 & 0.70 & 0.62 & 0.64 & 0.12 \\
\multirow{2}{*}{Gemma 7B (it)} & Num. & \cellcolor{cyan!10.1} 0.04 & 0.22 & 0.71 & 0.60 & 0.66 & 0.20 \\
 & Q\&A & \cellcolor{orange!10.1} 0.36 & 0.38 & 0.59 & 0.58 & 0.59 & 0.44 \\
\multirow{2}{*}{Gemma 2B (it)} & Num. & 0.12 & 0.27 & \cellcolor{orange!2.6} 0.46 & \cellcolor{orange!23.6} 0.46 & \cellcolor{orange!12.7} 0.50 & 0.05 \\
 & Q\&A & \cellcolor{orange!25.0} 0.38 & \cellcolor{orange!25.0} 0.41 & \cellcolor{orange!25.0} 0.42 & \cellcolor{orange!17.9} 0.46 & \cellcolor{orange!25.0} 0.48 & 0.23 \\
\multirow{2}{*}{Gemma 7B} & Num. & \cellcolor{orange!6.0} 0.35 & \cellcolor{orange!1.6} 0.38 & 0.50 & 0.51 & 0.52 & 0.22 \\
 & Q\&A & 0.15 & 0.25 & 0.65 & \cellcolor{orange!8.0} 0.48 & 0.63 & 0.13 \\
\multirow{2}{*}{Gemma 2B} & Num. & \cellcolor{cyan!25.0} 0.01 & 0.23 & 0.57 & 0.53 & \cellcolor{orange!11.9} 0.50 & 0.12 \\
 & Q\&A & \cellcolor{cyan!24.3} 0.01 & 0.24 & 0.63 & 0.54 & 0.61 & 0.03 \\
\midrule
LR & - & 0.02 & 0.15 & 0.86 & 0.78 & - & - \\
% GBM & - & 0.00 & 0.12 & 0.91 & 0.83 & - & - \\
XGBoost & - & 0.00 & 0.12 & 0.91 & 0.83 & - & - \\
\bottomrule
\end{tabular}


==> tables/both_prompting_schemes_different_rows/acsemployment_sorted_by_size.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\shortstack{Prompting\\ scheme}}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{ROC \\ AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
\multirow{2}{*}{GPT 4o mini (it)} & Num. & 0.23 & 0.23 & 0.80 & 0.73 & \cellcolor{cyan!0.3} 0.77 & 0.28 \\
 & Q\&A & 0.28 & 0.29 & 0.79 & 0.65 & 0.74 & 0.41 \\
\multirow{2}{*}{Llama 3 70B (it)} & Num. & \cellcolor{cyan!2.6} 0.05 & \cellcolor{cyan!25.0} 0.14 & \cellcolor{cyan!25.0} 0.88 & \cellcolor{cyan!25.0} 0.81 & \cellcolor{cyan!25.0} 0.81 & 0.32 \\
 & Q\&A & 0.17 & 0.19 & \cellcolor{cyan!13.5} 0.85 & 0.73 & \cellcolor{cyan!8.0} 0.78 & 0.29 \\
\multirow{2}{*}{Llama 3 70B} & Num. & \cellcolor{cyan!1.9} 0.05 & \cellcolor{cyan!17.5} 0.15 & \cellcolor{cyan!14.6} 0.86 & \cellcolor{cyan!5.9} 0.78 & \cellcolor{cyan!4.2} 0.78 & 0.31 \\
 & Q\&A & 0.25 & 0.26 & 0.82 & 0.52 & 0.74 & 0.12 \\
\multirow{2}{*}{Mixtral 8x22B (it)} & Num. & 0.06 & \cellcolor{cyan!22.2} 0.14 & \cellcolor{cyan!24.5} 0.87 & \cellcolor{cyan!16.5} 0.79 & \cellcolor{cyan!21.1} 0.80 & 0.33 \\
 & Q\&A & \cellcolor{orange!23.0} 0.38 & \cellcolor{orange!11.0} 0.39 & 0.60 & 0.51 & 0.60 & 0.26 \\
\multirow{2}{*}{Mistral 8x22B} & Num. & 0.15 & 0.18 & 0.82 & \cellcolor{cyan!20.8} 0.80 & \cellcolor{cyan!15.7} 0.79 & 0.35 \\
 & Q\&A & 0.21 & 0.24 & \cellcolor{cyan!15.2} 0.86 & 0.52 & \cellcolor{cyan!3.4} 0.78 & 0.08 \\
\multirow{2}{*}{Yi 34B (it)} & Num. & 0.15 & 0.21 & 0.81 & 0.51 & \cellcolor{cyan!13.4} 0.79 & 0.18 \\
 & Q\&A & 0.14 & 0.21 & 0.79 & 0.69 & 0.73 & 0.20 \\
\multirow{2}{*}{Yi 34B} & Num. & 0.13 & 0.23 & 0.66 & 0.50 & 0.64 & 0.11 \\
 & Q\&A & 0.08 & 0.23 & 0.70 & 0.62 & 0.64 & 0.12 \\
\multirow{2}{*}{Mixtral 8x7B (it)} & Num. & 0.07 & \cellcolor{cyan!17.5} 0.15 & \cellcolor{cyan!23.4} 0.87 & \cellcolor{cyan!7.3} 0.78 & \cellcolor{cyan!8.0} 0.78 & 0.27 \\
 & Q\&A & 0.22 & 0.24 & 0.82 & 0.73 & 0.75 & 0.44 \\
\multirow{2}{*}{Mistral 8x7B} & Num. & 0.08 & 0.17 & 0.81 & 0.73 & 0.75 & 0.25 \\
 & Q\&A & 0.30 & 0.31 & 0.81 & \cellcolor{orange!24.3} 0.45 & 0.74 & 0.06 \\
\multirow{2}{*}{Mistral 7B (it)} & Num. & \cellcolor{cyan!8.7} 0.04 & 0.19 & 0.79 & 0.69 & 0.76 & 0.27 \\
 & Q\&A & \cellcolor{orange!6.7} 0.35 & 0.36 & 0.72 & 0.63 & 0.66 & 0.49 \\
\multirow{2}{*}{Llama 3 8B (it)} & Num. & 0.08 & \cellcolor{cyan!0.7} 0.17 & 0.82 & 0.77 & 0.77 & 0.29 \\
 & Q\&A & 0.07 & 0.19 & 0.79 & 0.74 & 0.74 & 0.22 \\
\multirow{2}{*}{Llama 3 8B} & Num. & 0.15 & 0.23 & 0.75 & \cellcolor{orange!23.6} 0.46 & 0.68 & 0.11 \\
 & Q\&A & 0.34 & 0.34 & 0.76 & \cellcolor{orange!25.0} 0.45 & 0.69 & 0.06 \\
\multirow{2}{*}{Mistral 7B} & Num. & 0.14 & 0.19 & 0.80 & \cellcolor{cyan!13.0} 0.79 & \cellcolor{cyan!11.9} 0.79 & 0.42 \\
 & Q\&A & 0.26 & 0.30 & 0.76 & \cellcolor{orange!25.0} 0.45 & 0.69 & 0.04 \\
\multirow{2}{*}{Gemma 7B (it)} & Num. & \cellcolor{cyan!10.1} 0.04 & 0.22 & 0.71 & 0.60 & 0.66 & 0.20 \\
 & Q\&A & \cellcolor{orange!10.1} 0.36 & 0.38 & 0.59 & 0.58 & 0.59 & 0.44 \\
\multirow{2}{*}{Gemma 2B (it)} & Num. & 0.12 & 0.27 & \cellcolor{orange!2.6} 0.46 & \cellcolor{orange!23.6} 0.46 & \cellcolor{orange!12.7} 0.50 & 0.05 \\
 & Q\&A & \cellcolor{orange!25.0} 0.38 & \cellcolor{orange!25.0} 0.41 & \cellcolor{orange!25.0} 0.42 & \cellcolor{orange!17.9} 0.46 & \cellcolor{orange!25.0} 0.48 & 0.23 \\
\multirow{2}{*}{Gemma 7B} & Num. & \cellcolor{orange!6.0} 0.35 & \cellcolor{orange!1.6} 0.38 & 0.50 & 0.51 & 0.52 & 0.22 \\
 & Q\&A & 0.15 & 0.25 & 0.65 & \cellcolor{orange!8.0} 0.48 & 0.63 & 0.13 \\
\multirow{2}{*}{Gemma 2B} & Num. & \cellcolor{cyan!25.0} 0.01 & 0.23 & 0.57 & 0.53 & \cellcolor{orange!11.9} 0.50 & 0.12 \\
 & Q\&A & \cellcolor{cyan!24.3} 0.01 & 0.24 & 0.63 & 0.54 & 0.61 & 0.03 \\
\midrule
LR & - & 0.02 & 0.15 & 0.86 & 0.78 & - & - \\
% GBM & - & 0.00 & 0.12 & 0.91 & 0.83 & - & - \\
XGBoost & - & 0.00 & 0.12 & 0.91 & 0.83 & - & - \\
\bottomrule
\end{tabular}


==> tables/both_prompting_schemes_different_rows/acsincome.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\shortstack{Prompting\\ scheme}}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{ROC \\ AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
\multirow{2}{*}{GPT 4o mini (it)} & Num. & \cellcolor{cyan!25.0} 0.05 & \cellcolor{cyan!25.0} 0.16 & \cellcolor{cyan!7.0} 0.83 & \cellcolor{cyan!22.0} 0.78 & \cellcolor{cyan!14.5} 0.78 & 0.32 \\
 & Q\&A & 0.24 & 0.24 & \cellcolor{cyan!20.2} 0.85 & 0.74 & \cellcolor{cyan!19.8} 0.78 & 0.48 \\
\multirow{2}{*}{Llama 3 70B (it)} & Num. & 0.25 & 0.23 & \cellcolor{cyan!8.4} 0.84 & 0.67 & 0.74 & 0.29 \\
 & Q\&A & 0.27 & 0.27 & \cellcolor{cyan!25.0} 0.86 & 0.69 & \cellcolor{cyan!13.2} 0.78 & 0.42 \\
\multirow{2}{*}{Llama 3 70B} & Num. & 0.27 & 0.24 & 0.82 & 0.54 & \cellcolor{cyan!25.0} 0.79 & 0.25 \\
 & Q\&A & 0.20 & \cellcolor{cyan!2.6} 0.20 & \cellcolor{cyan!22.2} 0.86 & 0.70 & \cellcolor{cyan!23.7} 0.78 & 0.14 \\
\multirow{2}{*}{Llama 3 8B (it)} & Num. & 0.23 & 0.23 & 0.81 & 0.67 & 0.67 & 0.16 \\
 & Q\&A & 0.32 & 0.30 & \cellcolor{cyan!17.4} 0.85 & 0.62 & 0.73 & 0.37 \\
\multirow{2}{*}{Llama 3 8B} & Num. & 0.14 & 0.24 & 0.63 & \cellcolor{orange!3.9} 0.40 & 0.65 & 0.07 \\
 & Q\&A & 0.25 & 0.26 & 0.81 & \cellcolor{orange!20.8} 0.38 & 0.70 & 0.05 \\
\multirow{2}{*}{Mixtral 8x22B (it)} & Num. & 0.11 & \cellcolor{cyan!20.7} 0.17 & \cellcolor{cyan!11.1} 0.84 & \cellcolor{cyan!16.5} 0.77 & \cellcolor{cyan!5.4} 0.77 & 0.30 \\
 & Q\&A & 0.21 & 0.22 & \cellcolor{cyan!16.0} 0.85 & \cellcolor{cyan!11.1} 0.76 & 0.75 & 0.48 \\
\multirow{2}{*}{Mixtral 8x22B} & Num. & 0.13 & \cellcolor{cyan!15.4} 0.18 & 0.82 & \cellcolor{cyan!0.2} 0.74 & \cellcolor{cyan!4.1} 0.77 & 0.38 \\
 & Q\&A & 0.17 & \cellcolor{cyan!9.0} 0.19 & \cellcolor{cyan!19.5} 0.85 & 0.68 & 0.74 & 0.10 \\
\multirow{2}{*}{Mixtral 8x7B (it)} & Num. & \cellcolor{cyan!3.1} 0.10 & \cellcolor{cyan!20.7} 0.17 & \cellcolor{cyan!9.1} 0.84 & \cellcolor{cyan!10.5} 0.76 & 0.73 & 0.28 \\
 & Q\&A & 0.16 & \cellcolor{cyan!12.2} 0.18 & \cellcolor{cyan!21.5} 0.86 & \cellcolor{cyan!25.0} 0.78 & \cellcolor{cyan!19.8} 0.78 & 0.42 \\
\multirow{2}{*}{Mixtral 8x7B} & Num. & \cellcolor{cyan!13.4} 0.07 & \cellcolor{cyan!19.7} 0.17 & 0.81 & \cellcolor{cyan!22.6} 0.78 & 0.74 & 0.28 \\
 & Q\&A & 0.17 & 0.21 & \cellcolor{cyan!0.8} 0.83 & 0.65 & 0.76 & 0.06 \\
\multirow{2}{*}{Mistral 7B (it)} & Num. & 0.16 & \cellcolor{cyan!5.8} 0.19 & \cellcolor{cyan!1.5} 0.83 & 0.70 & 0.76 & 0.20 \\
 & Q\&A & 0.21 & 0.22 & \cellcolor{cyan!4.2} 0.83 & \cellcolor{cyan!16.5} 0.77 & \cellcolor{cyan!0.1} 0.77 & 0.42 \\
\multirow{2}{*}{Mistral 7B} & Num. & 0.36 & 0.32 & 0.75 & 0.49 & 0.70 & 0.35 \\
 & Q\&A & 0.20 & 0.23 & 0.80 & 0.73 & 0.74 & 0.04 \\
\multirow{2}{*}{Yi 34B (it)} & Num. & 0.22 & 0.21 & 0.80 & 0.48 & \cellcolor{cyan!9.3} 0.77 & 0.20 \\
 & Q\&A & 0.19 & \cellcolor{cyan!6.3} 0.19 & \cellcolor{cyan!21.5} 0.86 & 0.72 & 0.74 & 0.34 \\
\multirow{2}{*}{Yi 34B} & Num. & 0.15 & \cellcolor{cyan!10.0} 0.19 & \cellcolor{cyan!4.2} 0.83 & 0.61 & 0.75 & 0.23 \\
 & Q\&A & 0.25 & 0.22 & \cellcolor{cyan!17.4} 0.85 & 0.62 & \cellcolor{cyan!2.7} 0.77 & 0.20 \\
\multirow{2}{*}{Gemma 7B (it)} & Num. & 0.33 & 0.30 & 0.78 & 0.42 & 0.63 & 0.14 \\
 & Q\&A & \cellcolor{orange!16.4} 0.61 & \cellcolor{orange!5.8} 0.59 & \cellcolor{cyan!11.1} 0.84 & \cellcolor{orange!25.0} 0.37 & 0.70 & 0.06 \\
\multirow{2}{*}{Gemma 2B (it)} & Num. & 0.28 & 0.31 & \cellcolor{orange!25.0} 0.50 & \cellcolor{orange!25.0} 0.37 & 0.63 & 0.00 \\
 & Q\&A & \cellcolor{orange!25.0} 0.63 & \cellcolor{orange!25.0} 0.63 & 0.73 & \cellcolor{orange!25.0} 0.37 & 0.63 & 0.00 \\
\multirow{2}{*}{Gemma 7B} & Num. & 0.15 & \cellcolor{cyan!2.6} 0.20 & 0.80 & 0.73 & 0.74 & 0.24 \\
 & Q\&A & 0.24 & 0.27 & 0.76 & \cellcolor{orange!25.0} 0.37 & 0.69 & 0.04 \\
\multirow{2}{*}{Gemma 2B} & Num. & 0.37 & 0.37 & \cellcolor{orange!25.0} 0.50 & 0.63 & 0.63 & 0.00 \\
 & Q\&A & 0.14 & 0.25 & 0.62 & 0.45 & \cellcolor{orange!25.0} 0.59 & 0.02 \\
\midrule
LR & - & 0.03 & 0.18 & 0.79 & 0.74 & - & - \\
% GBM & - & 0.01 & 0.13 & 0.89 & 0.81 & - & - \\
XGBoost & - & 0.00 & 0.13 & 0.90 & 0.82 & - & - \\
\bottomrule
\end{tabular}


==> tables/both_prompting_schemes_different_rows/acsincome_sorted_by_size.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\shortstack{Prompting\\ scheme}}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{ROC \\ AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
\multirow{2}{*}{GPT 4o mini (it)} & Num. & \cellcolor{cyan!25.0} 0.05 & \cellcolor{cyan!25.0} 0.16 & \cellcolor{cyan!7.0} 0.83 & \cellcolor{cyan!22.0} 0.78 & \cellcolor{cyan!14.5} 0.78 & 0.32 \\
 & Q\&A & 0.24 & 0.24 & \cellcolor{cyan!20.2} 0.85 & 0.74 & \cellcolor{cyan!19.8} 0.78 & 0.48 \\
\multirow{2}{*}{Llama 3 70B (it)} & Num. & 0.25 & 0.23 & \cellcolor{cyan!8.4} 0.84 & 0.67 & 0.74 & 0.29 \\
 & Q\&A & 0.27 & 0.27 & \cellcolor{cyan!25.0} 0.86 & 0.69 & \cellcolor{cyan!13.2} 0.78 & 0.42 \\
\multirow{2}{*}{Llama 3 70B} & Num. & 0.27 & 0.24 & 0.82 & 0.54 & \cellcolor{cyan!25.0} 0.79 & 0.25 \\
 & Q\&A & 0.20 & \cellcolor{cyan!2.6} 0.20 & \cellcolor{cyan!22.2} 0.86 & 0.70 & \cellcolor{cyan!23.7} 0.78 & 0.14 \\
\multirow{2}{*}{Mixtral 8x22B (it)} & Num. & 0.11 & \cellcolor{cyan!20.7} 0.17 & \cellcolor{cyan!11.1} 0.84 & \cellcolor{cyan!16.5} 0.77 & \cellcolor{cyan!5.4} 0.77 & 0.30 \\
 & Q\&A & 0.21 & 0.22 & \cellcolor{cyan!16.0} 0.85 & \cellcolor{cyan!11.1} 0.76 & 0.75 & 0.48 \\
\multirow{2}{*}{Mixtral 8x22B} & Num. & 0.13 & \cellcolor{cyan!15.4} 0.18 & 0.82 & \cellcolor{cyan!0.2} 0.74 & \cellcolor{cyan!4.1} 0.77 & 0.38 \\
 & Q\&A & 0.17 & \cellcolor{cyan!9.0} 0.19 & \cellcolor{cyan!19.5} 0.85 & 0.68 & 0.74 & 0.10 \\
\multirow{2}{*}{Yi 34B (it)} & Num. & 0.22 & 0.21 & 0.80 & 0.48 & \cellcolor{cyan!9.3} 0.77 & 0.20 \\
 & Q\&A & 0.19 & \cellcolor{cyan!6.3} 0.19 & \cellcolor{cyan!21.5} 0.86 & 0.72 & 0.74 & 0.34 \\
\multirow{2}{*}{Yi 34B} & Num. & 0.15 & \cellcolor{cyan!10.0} 0.19 & \cellcolor{cyan!4.2} 0.83 & 0.61 & 0.75 & 0.23 \\
 & Q\&A & 0.25 & 0.22 & \cellcolor{cyan!17.4} 0.85 & 0.62 & \cellcolor{cyan!2.7} 0.77 & 0.20 \\
\multirow{2}{*}{Mixtral 8x7B (it)} & Num. & \cellcolor{cyan!3.1} 0.10 & \cellcolor{cyan!20.7} 0.17 & \cellcolor{cyan!9.1} 0.84 & \cellcolor{cyan!10.5} 0.76 & 0.73 & 0.28 \\
 & Q\&A & 0.16 & \cellcolor{cyan!12.2} 0.18 & \cellcolor{cyan!21.5} 0.86 & \cellcolor{cyan!25.0} 0.78 & \cellcolor{cyan!19.8} 0.78 & 0.42 \\
\multirow{2}{*}{Mixtral 8x7B} & Num. & \cellcolor{cyan!13.4} 0.07 & \cellcolor{cyan!19.7} 0.17 & 0.81 & \cellcolor{cyan!22.6} 0.78 & 0.74 & 0.28 \\
 & Q\&A & 0.17 & 0.21 & \cellcolor{cyan!0.8} 0.83 & 0.65 & 0.76 & 0.06 \\
\multirow{2}{*}{Llama 3 8B (it)} & Num. & 0.23 & 0.23 & 0.81 & 0.67 & 0.67 & 0.16 \\
 & Q\&A & 0.32 & 0.30 & \cellcolor{cyan!17.4} 0.85 & 0.62 & 0.73 & 0.37 \\
\multirow{2}{*}{Llama 3 8B} & Num. & 0.14 & 0.24 & 0.63 & \cellcolor{orange!3.9} 0.40 & 0.65 & 0.07 \\
 & Q\&A & 0.25 & 0.26 & 0.81 & \cellcolor{orange!20.8} 0.38 & 0.70 & 0.05 \\
\multirow{2}{*}{Mistral 7B (it)} & Num. & 0.16 & \cellcolor{cyan!5.8} 0.19 & \cellcolor{cyan!1.5} 0.83 & 0.70 & 0.76 & 0.20 \\
 & Q\&A & 0.21 & 0.22 & \cellcolor{cyan!4.2} 0.83 & \cellcolor{cyan!16.5} 0.77 & \cellcolor{cyan!0.1} 0.77 & 0.42 \\
\multirow{2}{*}{Mistral 7B} & Num. & 0.36 & 0.32 & 0.75 & 0.49 & 0.70 & 0.35 \\
 & Q\&A & 0.20 & 0.23 & 0.80 & 0.73 & 0.74 & 0.04 \\
\multirow{2}{*}{Gemma 7B (it)} & Num. & 0.33 & 0.30 & 0.78 & 0.42 & 0.63 & 0.14 \\
 & Q\&A & \cellcolor{orange!16.4} 0.61 & \cellcolor{orange!5.8} 0.59 & \cellcolor{cyan!11.1} 0.84 & \cellcolor{orange!25.0} 0.37 & 0.70 & 0.06 \\
\multirow{2}{*}{Gemma 2B (it)} & Num. & 0.28 & 0.31 & \cellcolor{orange!25.0} 0.50 & \cellcolor{orange!25.0} 0.37 & 0.63 & 0.00 \\
 & Q\&A & \cellcolor{orange!25.0} 0.63 & \cellcolor{orange!25.0} 0.63 & 0.73 & \cellcolor{orange!25.0} 0.37 & 0.63 & 0.00 \\
\multirow{2}{*}{Gemma 7B} & Num. & 0.15 & \cellcolor{cyan!2.6} 0.20 & 0.80 & 0.73 & 0.74 & 0.24 \\
 & Q\&A & 0.24 & 0.27 & 0.76 & \cellcolor{orange!25.0} 0.37 & 0.69 & 0.04 \\
\multirow{2}{*}{Gemma 2B} & Num. & 0.37 & 0.37 & \cellcolor{orange!25.0} 0.50 & 0.63 & 0.63 & 0.00 \\
 & Q\&A & 0.14 & 0.25 & 0.62 & 0.45 & \cellcolor{orange!25.0} 0.59 & 0.02 \\
\midrule
LR & - & 0.03 & 0.18 & 0.79 & 0.74 & - & - \\
% GBM & - & 0.01 & 0.13 & 0.89 & 0.81 & - & - \\
XGBoost & - & 0.00 & 0.13 & 0.90 & 0.82 & - & - \\
\bottomrule
\end{tabular}


==> tables/both_prompting_schemes_different_rows/acsmobility.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\shortstack{Prompting\\ scheme}}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{ROC \\ AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
\multirow{2}{*}{GPT 4o mini (it)} & Num. & 0.22 & 0.25 & \cellcolor{orange!0.2} 0.49 & \cellcolor{cyan!25.0} 0.73 & 0.62 & 0.09 \\
 & Q\&A & 0.26 & 0.26 & \cellcolor{cyan!5.2} 0.57 & \cellcolor{cyan!25.0} 0.73 & 0.67 & 0.02 \\
\multirow{2}{*}{Llama 3 70B (it)} & Num. & \cellcolor{cyan!12.1} 0.05 & \cellcolor{cyan!23.1} 0.20 & 0.52 & \cellcolor{cyan!25.0} 0.73 & 0.52 & 0.08 \\
 & Q\&A & 0.20 & \cellcolor{cyan!0.2} 0.25 & 0.57 & 0.58 & 0.63 & 0.18 \\
\multirow{2}{*}{Llama 3 70B} & Num. & \cellcolor{cyan!8.6} 0.06 & \cellcolor{cyan!22.7} 0.20 & 0.53 & \cellcolor{cyan!20.7} 0.73 & 0.48 & 0.08 \\
 & Q\&A & 0.22 & \cellcolor{cyan!3.5} 0.24 & 0.55 & 0.53 & 0.49 & 0.04 \\
\multirow{2}{*}{Llama 3 8B (it)} & Num. & 0.11 & \cellcolor{cyan!18.9} 0.21 & \cellcolor{orange!2.7} 0.49 & \cellcolor{cyan!23.4} 0.73 & 0.67 & 0.06 \\
 & Q\&A & 0.15 & \cellcolor{cyan!12.4} 0.22 & 0.56 & \cellcolor{cyan!5.3} 0.70 & 0.54 & 0.17 \\
\multirow{2}{*}{Llama 3 8B} & Num. & 0.14 & \cellcolor{cyan!15.7} 0.21 & 0.51 & \cellcolor{cyan!19.1} 0.72 & 0.64 & 0.09 \\
 & Q\&A & 0.10 & \cellcolor{cyan!20.3} 0.20 & 0.55 & \cellcolor{cyan!24.5} 0.73 & 0.50 & 0.04 \\
\multirow{2}{*}{Mixtral 8x22B (it)} & Num. & \cellcolor{cyan!11.7} 0.05 & \cellcolor{cyan!24.1} 0.20 & 0.54 & \cellcolor{cyan!25.0} 0.73 & 0.47 & 0.05 \\
 & Q\&A & 0.40 & 0.40 & 0.51 & 0.39 & 0.53 & 0.24 \\
\multirow{2}{*}{Mistral 8x22B} & Num. & 0.13 & \cellcolor{cyan!12.9} 0.22 & 0.49 & \cellcolor{cyan!25.0} 0.73 & 0.40 & 0.09 \\
 & Q\&A & 0.11 & \cellcolor{cyan!19.9} 0.21 & 0.55 & \cellcolor{cyan!25.0} 0.73 & 0.62 & 0.02 \\
\multirow{2}{*}{Mixtral 8x7B (it)} & Num. & 0.11 & \cellcolor{cyan!19.4} 0.21 & 0.51 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!22.8} 0.73 & 0.02 \\
 & Q\&A & 0.26 & 0.26 & \cellcolor{cyan!15.1} 0.58 & \cellcolor{cyan!25.0} 0.73 & 0.64 & 0.02 \\
\multirow{2}{*}{Mistral 8x7B} & Num. & 0.24 & 0.25 & \cellcolor{orange!25.0} 0.48 & \cellcolor{cyan!25.0} 0.73 & 0.47 & 0.03 \\
 & Q\&A & 0.14 & \cellcolor{cyan!17.5} 0.21 & 0.57 & \cellcolor{cyan!25.0} 0.73 & 0.57 & 0.03 \\
\multirow{2}{*}{Mistral 7B (it)} & Num. & 0.17 & \cellcolor{cyan!9.1} 0.23 & \cellcolor{orange!2.7} 0.49 & \cellcolor{cyan!24.5} 0.73 & \cellcolor{cyan!1.9} 0.69 & 0.07 \\
 & Q\&A & 0.26 & 0.26 & 0.57 & \cellcolor{cyan!25.0} 0.73 & 0.54 & 0.02 \\
\multirow{2}{*}{Mistral 7B} & Num. & 0.27 & 0.27 & 0.50 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!25.0} 0.73 & 0.00 \\
 & Q\&A & 0.20 & \cellcolor{cyan!7.2} 0.23 & 0.53 & \cellcolor{cyan!23.4} 0.73 & 0.34 & 0.01 \\
\multirow{2}{*}{Yi 34B (it)} & Num. & 0.23 & 0.25 & 0.50 & \cellcolor{orange!25.0} 0.27 & \cellcolor{cyan!25.0} 0.73 & 0.00 \\
 & Q\&A & 0.09 & \cellcolor{cyan!21.7} 0.20 & 0.56 & \cellcolor{cyan!15.4} 0.72 & 0.59 & 0.15 \\
\multirow{2}{*}{Yi 34B} & Num. & 0.15 & \cellcolor{cyan!9.6} 0.23 & 0.52 & 0.44 & 0.44 & 0.12 \\
 & Q\&A & \cellcolor{cyan!5.8} 0.07 & \cellcolor{cyan!23.6} 0.20 & 0.57 & \cellcolor{cyan!20.7} 0.73 & 0.66 & 0.08 \\
\multirow{2}{*}{Gemma 7B (it)} & Num. & 0.25 & 0.26 & \cellcolor{orange!12.6} 0.49 & \cellcolor{cyan!22.3} 0.73 & \cellcolor{cyan!22.3} 0.73 & 0.08 \\
& Q\&A & 0.25 & 0.26 & \cellcolor{cyan!25.0} 0.58 & \cellcolor{cyan!21.8} 0.73 & 0.68 & 0.11 \\
\multirow{2}{*}{Gemma 2B (it)} & Num. & \cellcolor{cyan!25.0} 0.02 & \cellcolor{cyan!25.0} 0.20 & 0.50 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{orange!25.0} 0.27 & 0.01 \\
 & Q\&A & \cellcolor{orange!25.0} 0.73 & \cellcolor{orange!25.0} 0.73 & 0.52 & \cellcolor{orange!25.0} 0.27 & 0.40 & 0.00 \\
\multirow{2}{*}{Gemma 7B} & Num. & 0.19 & \cellcolor{cyan!5.8} 0.24 & 0.49 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!25.0} 0.73 & 0.06 \\
 & Q\&A & 0.41 & 0.37 & 0.50 & \cellcolor{orange!25.0} 0.27 & 0.41 & 0.10 \\
\multirow{2}{*}{Gemma 2B} & Num. & 0.27 & 0.27 & 0.50 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!25.0} 0.73 & 0.00 \\
 & Q\&A & 0.25 & 0.26 & 0.51 & 0.34 & 0.48 & 0.02 \\
\midrule
LR & - & 0.02 & 0.19 & 0.61 & 0.74 & - & - \\
% GBM & - & 0.01 & 0.17 & 0.74 & 0.76 & - & - \\
XGBoost & - & 0.00 & 0.16 & 0.74 & 0.76 & - & - \\
\bottomrule
\end{tabular}


==> tables/both_prompting_schemes_different_rows/acsmobility_sorted_by_size.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\shortstack{Prompting\\ scheme}}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{ROC \\ AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
\multirow{2}{*}{GPT 4o mini (it)} & Num. & 0.22 & 0.25 & \cellcolor{orange!0.2} 0.49 & \cellcolor{cyan!25.0} 0.73 & 0.62 & 0.09 \\
 & Q\&A & 0.26 & 0.26 & \cellcolor{cyan!5.2} 0.57 & \cellcolor{cyan!25.0} 0.73 & 0.67 & 0.02 \\
\multirow{2}{*}{Llama 3 70B (it)} & Num. & \cellcolor{cyan!12.1} 0.05 & \cellcolor{cyan!23.1} 0.20 & 0.52 & \cellcolor{cyan!25.0} 0.73 & 0.52 & 0.08 \\
 & Q\&A & 0.20 & \cellcolor{cyan!0.2} 0.25 & 0.57 & 0.58 & 0.63 & 0.18 \\
\multirow{2}{*}{Llama 3 70B} & Num. & \cellcolor{cyan!8.6} 0.06 & \cellcolor{cyan!22.7} 0.20 & 0.53 & \cellcolor{cyan!20.7} 0.73 & 0.48 & 0.08 \\
 & Q\&A & 0.22 & \cellcolor{cyan!3.5} 0.24 & 0.55 & 0.53 & 0.49 & 0.04 \\
\multirow{2}{*}{Mixtral 8x22B (it)} & Num. & \cellcolor{cyan!11.7} 0.05 & \cellcolor{cyan!24.1} 0.20 & 0.54 & \cellcolor{cyan!25.0} 0.73 & 0.47 & 0.05 \\
 & Q\&A & 0.40 & 0.40 & 0.51 & 0.39 & 0.53 & 0.24 \\
\multirow{2}{*}{Mistral 8x22B} & Num. & 0.13 & \cellcolor{cyan!12.9} 0.22 & 0.49 & \cellcolor{cyan!25.0} 0.73 & 0.40 & 0.09 \\
 & Q\&A & 0.11 & \cellcolor{cyan!19.9} 0.21 & 0.55 & \cellcolor{cyan!25.0} 0.73 & 0.62 & 0.02 \\
\multirow{2}{*}{Yi 34B (it)} & Num. & 0.23 & 0.25 & 0.50 & \cellcolor{orange!25.0} 0.27 & \cellcolor{cyan!25.0} 0.73 & 0.00 \\
 & Q\&A & 0.09 & \cellcolor{cyan!21.7} 0.20 & 0.56 & \cellcolor{cyan!15.4} 0.72 & 0.59 & 0.15 \\
\multirow{2}{*}{Yi 34B} & Num. & 0.15 & \cellcolor{cyan!9.6} 0.23 & 0.52 & 0.44 & 0.44 & 0.12 \\
 & Q\&A & \cellcolor{cyan!5.8} 0.07 & \cellcolor{cyan!23.6} 0.20 & 0.57 & \cellcolor{cyan!20.7} 0.73 & 0.66 & 0.08 \\
\multirow{2}{*}{Mixtral 8x7B (it)} & Num. & 0.11 & \cellcolor{cyan!19.4} 0.21 & 0.51 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!22.8} 0.73 & 0.02 \\
 & Q\&A & 0.26 & 0.26 & \cellcolor{cyan!15.1} 0.58 & \cellcolor{cyan!25.0} 0.73 & 0.64 & 0.02 \\
\multirow{2}{*}{Mistral 8x7B} & Num. & 0.24 & 0.25 & \cellcolor{orange!25.0} 0.48 & \cellcolor{cyan!25.0} 0.73 & 0.47 & 0.03 \\
 & Q\&A & 0.14 & \cellcolor{cyan!17.5} 0.21 & 0.57 & \cellcolor{cyan!25.0} 0.73 & 0.57 & 0.03 \\
\multirow{2}{*}{Llama 3 8B (it)} & Num. & 0.11 & \cellcolor{cyan!18.9} 0.21 & \cellcolor{orange!2.7} 0.49 & \cellcolor{cyan!23.4} 0.73 & 0.67 & 0.06 \\
 & Q\&A & 0.15 & \cellcolor{cyan!12.4} 0.22 & 0.56 & \cellcolor{cyan!5.3} 0.70 & 0.54 & 0.17 \\
\multirow{2}{*}{Llama 3 8B} & Num. & 0.14 & \cellcolor{cyan!15.7} 0.21 & 0.51 & \cellcolor{cyan!19.1} 0.72 & 0.64 & 0.09 \\
 & Q\&A & 0.10 & \cellcolor{cyan!20.3} 0.20 & 0.55 & \cellcolor{cyan!24.5} 0.73 & 0.50 & 0.04 \\
\multirow{2}{*}{Mistral 7B (it)} & Num. & 0.17 & \cellcolor{cyan!9.1} 0.23 & \cellcolor{orange!2.7} 0.49 & \cellcolor{cyan!24.5} 0.73 & \cellcolor{cyan!1.9} 0.69 & 0.07 \\
 & Q\&A & 0.26 & 0.26 & 0.57 & \cellcolor{cyan!25.0} 0.73 & 0.54 & 0.02 \\
\multirow{2}{*}{Mistral 7B} & Num. & 0.27 & 0.27 & 0.50 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!25.0} 0.73 & 0.00 \\
 & Q\&A & 0.20 & \cellcolor{cyan!7.2} 0.23 & 0.53 & \cellcolor{cyan!23.4} 0.73 & 0.34 & 0.01 \\
\multirow{2}{*}{Gemma 7B (it)} & Num. & 0.25 & 0.26 & \cellcolor{orange!12.6} 0.49 & \cellcolor{cyan!22.3} 0.73 & \cellcolor{cyan!22.3} 0.73 & 0.08 \\
& Q\&A & 0.25 & 0.26 & \cellcolor{cyan!25.0} 0.58 & \cellcolor{cyan!21.8} 0.73 & 0.68 & 0.11 \\
\multirow{2}{*}{Gemma 2B (it)} & Num. & \cellcolor{cyan!25.0} 0.02 & \cellcolor{cyan!25.0} 0.20 & 0.50 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{orange!25.0} 0.27 & 0.01 \\
 & Q\&A & \cellcolor{orange!25.0} 0.73 & \cellcolor{orange!25.0} 0.73 & 0.52 & \cellcolor{orange!25.0} 0.27 & 0.40 & 0.00 \\
\multirow{2}{*}{Gemma 7B} & Num. & 0.19 & \cellcolor{cyan!5.8} 0.24 & 0.49 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!25.0} 0.73 & 0.06 \\
 & Q\&A & 0.41 & 0.37 & 0.50 & \cellcolor{orange!25.0} 0.27 & 0.41 & 0.10 \\
\multirow{2}{*}{Gemma 2B} & Num. & 0.27 & 0.27 & 0.50 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!25.0} 0.73 & 0.00 \\
 & Q\&A & 0.25 & 0.26 & 0.51 & 0.34 & 0.48 & 0.02 \\
\midrule
LR & - & 0.02 & 0.19 & 0.61 & 0.74 & - & - \\
% GBM & - & 0.01 & 0.17 & 0.74 & 0.76 & - & - \\
XGBoost & - & 0.00 & 0.16 & 0.74 & 0.76 & - & - \\
\bottomrule
\end{tabular}


==> tables/both_prompting_schemes_different_rows/acspubliccoverage.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\shortstack{Prompting\\ scheme}}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{ROC \\ AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
\multirow{2}{*}{GPT 4o mini (it)} & Num. & 0.10 & \cellcolor{cyan!17.3} 0.20 & 0.68 & \cellcolor{cyan!17.8} 0.73 & 0.61 & 0.26 \\
 & Q\&A & 0.33 & 0.34 & \cellcolor{cyan!15.1} 0.71 & 0.60 & \cellcolor{cyan!5.8} 0.71 & 0.43 \\
\multirow{2}{*}{Llama 3 70B (it)} & Num. & 0.13 & \cellcolor{cyan!17.7} 0.20 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!24.4} 0.75 & \cellcolor{cyan!25.0} 0.75 & 0.23 \\
 & Q\&A & 0.16 & \cellcolor{cyan!12.9} 0.21 & 0.69 & \cellcolor{cyan!23.9} 0.75 & 0.52 & 0.20 \\
\multirow{2}{*}{Llama 3 70B} & Num. & 0.12 & \cellcolor{cyan!12.4} 0.21 & 0.64 & 0.53 & 0.51 & 0.20 \\
 & Q\&A & 0.18 & \cellcolor{cyan!5.2} 0.22 & 0.67 & 0.63 & \cellcolor{cyan!20.9} 0.74 & 0.07 \\
\multirow{2}{*}{Llama 3 8B (it)} & Num. & 0.17 & \cellcolor{cyan!6.6} 0.22 & 0.64 & 0.68 & 0.69 & 0.09 \\
 & Q\&A & 0.11 & \cellcolor{cyan!9.5} 0.21 & 0.59 & \cellcolor{cyan!6.7} 0.71 & \cellcolor{cyan!1.7} 0.71 & 0.19 \\
\multirow{2}{*}{Llama 3 8B} & Num. & 0.20 & 0.25 & 0.51 & \cellcolor{orange!0.6} 0.34 & \cellcolor{orange!11.0} 0.34 & 0.07 \\
 & Q\&A & 0.41 & 0.38 & 0.55 & \cellcolor{orange!25.0} 0.30 & 0.50 & 0.02 \\
\multirow{2}{*}{Mixtral 8x22B (it)} & Num. & \cellcolor{cyan!25.0} 0.04 & \cellcolor{cyan!25.0} 0.18 & \cellcolor{cyan!11.0} 0.71 & \cellcolor{cyan!25.0} 0.75 & 0.57 & 0.21 \\
 & Q\&A & 0.24 & 0.25 & \cellcolor{cyan!3.5} 0.70 & \cellcolor{cyan!11.7} 0.72 & 0.69 & 0.17 \\
\multirow{2}{*}{Mistral 8x22B} & Num. & 0.29 & 0.29 & 0.54 & \cellcolor{cyan!1.1} 0.70 & \cellcolor{cyan!1.7} 0.71 & 0.06 \\
 & Q\&A & 0.32 & 0.30 & 0.59 & \cellcolor{orange!25.0} 0.30 & 0.56 & 0.05 \\
\multirow{2}{*}{Mixtral 8x7B (it)} & Num. & \cellcolor{cyan!15.2} 0.06 & \cellcolor{cyan!23.5} 0.19 & 0.69 & \cellcolor{cyan!22.2} 0.74 & 0.60 & 0.13 \\
 & Q\&A & 0.20 & \cellcolor{cyan!4.2} 0.23 & \cellcolor{cyan!4.4} 0.70 & \cellcolor{cyan!22.2} 0.74 & \cellcolor{cyan!10.5} 0.72 & 0.35 \\
\multirow{2}{*}{Mistral 8x7B} & Num. & 0.20 & 0.25 & 0.56 & 0.70 & \cellcolor{cyan!11.0} 0.72 & 0.07 \\
 & Q\&A & 0.41 & 0.37 & 0.57 & \cellcolor{orange!25.0} 0.30 & 0.38 & 0.03 \\
\multirow{2}{*}{Mistral 7B (it)} & Num. & \cellcolor{cyan!11.5} 0.07 & \cellcolor{cyan!14.8} 0.20 & 0.67 & 0.65 & 0.65 & 0.20 \\
 & Q\&A & 0.30 & 0.30 & 0.61 & 0.70 & 0.68 & 0.01 \\
\multirow{2}{*}{Mistral 7B} & Num. & 0.30 & 0.30 & 0.50 & \cellcolor{cyan!0.6} 0.70 & 0.70 & 0.05 \\
 & Q\&A & 0.29 & 0.30 & \cellcolor{orange!2.7} 0.45 & \cellcolor{orange!25.0} 0.30 & 0.70 & 0.02 \\
\multirow{2}{*}{Yi 34B (it)} & Num. & 0.22 & 0.24 & 0.57 & \cellcolor{orange!18.9} 0.31 & \cellcolor{cyan!1.7} 0.71 & 0.07 \\
 & Q\&A & \cellcolor{cyan!15.2} 0.06 & \cellcolor{cyan!21.6} 0.19 & 0.67 & \cellcolor{cyan!18.3} 0.74 & 0.70 & 0.13 \\
\multirow{2}{*}{Yi 34B} & Num. & \cellcolor{cyan!4.3} 0.09 & \cellcolor{cyan!17.7} 0.20 & 0.67 & 0.64 & 0.64 & 0.15 \\
 & Q\&A & \cellcolor{cyan!23.5} 0.04 & \cellcolor{cyan!13.9} 0.21 & 0.59 & \cellcolor{cyan!1.1} 0.70 & 0.56 & 0.07 \\
\multirow{2}{*}{Gemma 7B (it)} & Num. & 0.18 & 0.24 & 0.57 & 0.61 & 0.61 & 0.22 \\
 & Q\&A & 0.30 & 0.34 & 0.46 & 0.50 & \cellcolor{orange!25.0} 0.32 & 0.32 \\
\multirow{2}{*}{Gemma 2B (it)} & Num. & 0.24 & 0.29 & \cellcolor{orange!25.0} 0.42 & 0.42 & 0.70 & 0.17 \\
 & Q\&A & \cellcolor{orange!25.0} 0.70 & \cellcolor{orange!25.0} 0.70 & 0.54 & \cellcolor{orange!25.0} 0.30 & \cellcolor{orange!18.0} 0.33 & 0.00 \\
\multirow{2}{*}{Gemma 7B} & Num. & 0.18 & 0.26 & 0.48 & 0.70 & 0.70 & 0.11 \\
 & Q\&A & 0.15 & \cellcolor{cyan!0.3} 0.23 & 0.49 & 0.49 & 0.37 & 0.10 \\
\multirow{2}{*}{Gemma 2B} & Num. & 0.30 & 0.30 & 0.50 & 0.70 & 0.70 & 0.02 \\
 & Q\&A & 0.26 & 0.28 & 0.54 & \cellcolor{orange!25.0} 0.30 & 0.62 & 0.01 \\
\midrule
LR & - & 0.03 & 0.19 & 0.70 & 0.72 & - & - \\
% GBM & - & 0.01 & 0.14 & 0.83 & 0.80 & - & - \\
XGBoost & - & 0.00 & 0.14 & 0.84 & 0.80 & - & - \\
\bottomrule
\end{tabular}


==> tables/both_prompting_schemes_different_rows/acspubliccoverage_sorted_by_size.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\shortstack{Prompting\\ scheme}}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{ROC \\ AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
\multirow{2}{*}{GPT 4o mini (it)} & Num. & 0.10 & \cellcolor{cyan!17.3} 0.20 & 0.68 & \cellcolor{cyan!17.8} 0.73 & 0.61 & 0.26 \\
 & Q\&A & 0.33 & 0.34 & \cellcolor{cyan!15.1} 0.71 & 0.60 & \cellcolor{cyan!5.8} 0.71 & 0.43 \\
\multirow{2}{*}{Llama 3 70B (it)} & Num. & 0.13 & \cellcolor{cyan!17.7} 0.20 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!24.4} 0.75 & \cellcolor{cyan!25.0} 0.75 & 0.23 \\
 & Q\&A & 0.16 & \cellcolor{cyan!12.9} 0.21 & 0.69 & \cellcolor{cyan!23.9} 0.75 & 0.52 & 0.20 \\
\multirow{2}{*}{Llama 3 70B} & Num. & 0.12 & \cellcolor{cyan!12.4} 0.21 & 0.64 & 0.53 & 0.51 & 0.20 \\
 & Q\&A & 0.18 & \cellcolor{cyan!5.2} 0.22 & 0.67 & 0.63 & \cellcolor{cyan!20.9} 0.74 & 0.07 \\
\multirow{2}{*}{Mixtral 8x22B (it)} & Num. & \cellcolor{cyan!25.0} 0.04 & \cellcolor{cyan!25.0} 0.18 & \cellcolor{cyan!11.0} 0.71 & \cellcolor{cyan!25.0} 0.75 & 0.57 & 0.21 \\
 & Q\&A & 0.24 & 0.25 & \cellcolor{cyan!3.5} 0.70 & \cellcolor{cyan!11.7} 0.72 & 0.69 & 0.17 \\
\multirow{2}{*}{Mistral 8x22B} & Num. & 0.29 & 0.29 & 0.54 & \cellcolor{cyan!1.1} 0.70 & \cellcolor{cyan!1.7} 0.71 & 0.06 \\
 & Q\&A & 0.32 & 0.30 & 0.59 & \cellcolor{orange!25.0} 0.30 & 0.56 & 0.05 \\
\multirow{2}{*}{Yi 34B (it)} & Num. & 0.22 & 0.24 & 0.57 & \cellcolor{orange!18.9} 0.31 & \cellcolor{cyan!1.7} 0.71 & 0.07 \\
 & Q\&A & \cellcolor{cyan!15.2} 0.06 & \cellcolor{cyan!21.6} 0.19 & 0.67 & \cellcolor{cyan!18.3} 0.74 & 0.70 & 0.13 \\
\multirow{2}{*}{Yi 34B} & Num. & \cellcolor{cyan!4.3} 0.09 & \cellcolor{cyan!17.7} 0.20 & 0.67 & 0.64 & 0.64 & 0.15 \\
 & Q\&A & \cellcolor{cyan!23.5} 0.04 & \cellcolor{cyan!13.9} 0.21 & 0.59 & \cellcolor{cyan!1.1} 0.70 & 0.56 & 0.07 \\
\multirow{2}{*}{Mixtral 8x7B (it)} & Num. & \cellcolor{cyan!15.2} 0.06 & \cellcolor{cyan!23.5} 0.19 & 0.69 & \cellcolor{cyan!22.2} 0.74 & 0.60 & 0.13 \\
 & Q\&A & 0.20 & \cellcolor{cyan!4.2} 0.23 & \cellcolor{cyan!4.4} 0.70 & \cellcolor{cyan!22.2} 0.74 & \cellcolor{cyan!10.5} 0.72 & 0.35 \\
\multirow{2}{*}{Mistral 8x7B} & Num. & 0.20 & 0.25 & 0.56 & 0.70 & \cellcolor{cyan!11.0} 0.72 & 0.07 \\
 & Q\&A & 0.41 & 0.37 & 0.57 & \cellcolor{orange!25.0} 0.30 & 0.38 & 0.03 \\
\multirow{2}{*}{Llama 3 8B (it)} & Num. & 0.17 & \cellcolor{cyan!6.6} 0.22 & 0.64 & 0.68 & 0.69 & 0.09 \\
 & Q\&A & 0.11 & \cellcolor{cyan!9.5} 0.21 & 0.59 & \cellcolor{cyan!6.7} 0.71 & \cellcolor{cyan!1.7} 0.71 & 0.19 \\
\multirow{2}{*}{Llama 3 8B} & Num. & 0.20 & 0.25 & 0.51 & \cellcolor{orange!0.6} 0.34 & \cellcolor{orange!11.0} 0.34 & 0.07 \\
 & Q\&A & 0.41 & 0.38 & 0.55 & \cellcolor{orange!25.0} 0.30 & 0.50 & 0.02 \\
\multirow{2}{*}{Mistral 7B (it)} & Num. & \cellcolor{cyan!11.5} 0.07 & \cellcolor{cyan!14.8} 0.20 & 0.67 & 0.65 & 0.65 & 0.20 \\
 & Q\&A & 0.30 & 0.30 & 0.61 & 0.70 & 0.68 & 0.01 \\
\multirow{2}{*}{Mistral 7B} & Num. & 0.30 & 0.30 & 0.50 & \cellcolor{cyan!0.6} 0.70 & 0.70 & 0.05 \\
 & Q\&A & 0.29 & 0.30 & \cellcolor{orange!2.7} 0.45 & \cellcolor{orange!25.0} 0.30 & 0.70 & 0.02 \\
\multirow{2}{*}{Gemma 7B (it)} & Num. & 0.18 & 0.24 & 0.57 & 0.61 & 0.61 & 0.22 \\
 & Q\&A & 0.30 & 0.34 & 0.46 & 0.50 & \cellcolor{orange!25.0} 0.32 & 0.32 \\
\multirow{2}{*}{Gemma 2B (it)} & Num. & 0.24 & 0.29 & \cellcolor{orange!25.0} 0.42 & 0.42 & 0.70 & 0.17 \\
 & Q\&A & \cellcolor{orange!25.0} 0.70 & \cellcolor{orange!25.0} 0.70 & 0.54 & \cellcolor{orange!25.0} 0.30 & \cellcolor{orange!18.0} 0.33 & 0.00 \\
\multirow{2}{*}{Gemma 7B} & Num. & 0.18 & 0.26 & 0.48 & 0.70 & 0.70 & 0.11 \\
 & Q\&A & 0.15 & \cellcolor{cyan!0.3} 0.23 & 0.49 & 0.49 & 0.37 & 0.10 \\
\multirow{2}{*}{Gemma 2B} & Num. & 0.30 & 0.30 & 0.50 & 0.70 & 0.70 & 0.02 \\
 & Q\&A & 0.26 & 0.28 & 0.54 & \cellcolor{orange!25.0} 0.30 & 0.62 & 0.01 \\
\midrule
LR & - & 0.03 & 0.19 & 0.70 & 0.72 & - & - \\
% GBM & - & 0.01 & 0.14 & 0.83 & 0.80 & - & - \\
XGBoost & - & 0.00 & 0.14 & 0.84 & 0.80 & - & - \\
\bottomrule
\end{tabular}


==> tables/both_prompting_schemes_different_rows/acstraveltime.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\shortstack{Prompting\\ scheme}}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{ROC \\ AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
\multirow{2}{*}{GPT 4o mini (it)} & Num. & 0.15 & 0.27 & 0.58 & 0.57 & 0.51 & 0.22 \\
 & Q\&A & 0.39 & 0.40 & 0.65 & 0.55 & 0.60 & 0.36 \\
\multirow{2}{*}{Llama 3 70B (it)} & Num. & 0.12 & \cellcolor{cyan!21.4} 0.24 & 0.64 & 0.53 & \cellcolor{cyan!22.9} 0.61 & 0.13 \\
 & Q\&A & 0.15 & \cellcolor{cyan!22.6} 0.24 & \cellcolor{cyan!25.0} 0.70 & \cellcolor{cyan!25.0} 0.60 & \cellcolor{cyan!16.5} 0.61 & 0.12 \\
\multirow{2}{*}{Llama 3 70B} & Num. & 0.08 & \cellcolor{cyan!11.8} 0.25 & 0.52 & 0.46 & 0.56 & 0.05 \\
 & Q\&A & 0.09 & \cellcolor{cyan!21.4} 0.24 & 0.67 & 0.55 & \cellcolor{cyan!16.5} 0.61 & 0.05 \\
\multirow{2}{*}{Llama 3 8B (it)} & Num. & 0.11 & \cellcolor{cyan!11.8} 0.25 & 0.56 & 0.56 & 0.52 & 0.06 \\
 & Q\&A & 0.19 & 0.28 & 0.60 & 0.57 & 0.57 & 0.11 \\
\multirow{2}{*}{Llama 3 8B} & Num. & 0.12 & 0.26 & \cellcolor{orange!25.0} 0.48 & \cellcolor{orange!25.0} 0.44 & 0.55 & 0.02 \\
 & Q\&A & 0.08 & \cellcolor{cyan!7.1} 0.25 & 0.53 & 0.56 & 0.52 & 0.03 \\
\multirow{2}{*}{Mixtral 8x22B (it)} & Num. & 0.12 & \cellcolor{cyan!22.6} 0.24 & 0.64 & \cellcolor{cyan!20.3} 0.59 & \cellcolor{cyan!25.0} 0.61 & 0.14 \\
 & Q\&A & 0.31 & 0.33 & 0.66 & \cellcolor{cyan!17.1} 0.59 & \cellcolor{cyan!8.1} 0.61 & 0.15 \\
\multirow{2}{*}{Mistral 8x22B} & Num. & 0.30 & 0.34 & 0.57 & 0.58 & 0.58 & 0.17 \\
 & Q\&A & 0.20 & 0.28 & 0.63 & \cellcolor{orange!25.0} 0.44 & 0.56 & 0.04 \\
\multirow{2}{*}{Mixtral 8x7B (it)} & Num. & 0.09 & \cellcolor{cyan!23.8} 0.24 & 0.61 & 0.57 & \cellcolor{orange!18.6} 0.50 & 0.11 \\
 & Q\&A & \cellcolor{orange!25.0} 0.45 & \cellcolor{orange!25.0} 0.45 & 0.66 & 0.52 & 0.55 & 0.29 \\
\multirow{2}{*}{Mistral 8x7B} & Num. & 0.07 & \cellcolor{cyan!15.4} 0.25 & 0.57 & 0.58 & 0.57 & 0.12 \\
 & Q\&A & 0.28 & 0.32 & 0.60 & \cellcolor{orange!25.0} 0.44 & 0.52 & 0.03 \\
\multirow{2}{*}{Mistral 7B (it)} & Num. & 0.11 & \cellcolor{cyan!10.6} 0.25 & 0.55 & 0.56 & \cellcolor{orange!18.6} 0.50 & 0.10 \\
 & Q\&A & \cellcolor{orange!3.5} 0.41 & 0.42 & 0.59 & 0.57 & 0.53 & 0.19 \\
\multirow{2}{*}{Mistral 7B} & Num. & \cellcolor{orange!20.2} 0.44 & \cellcolor{orange!14.2} 0.44 & \cellcolor{orange!0.7} 0.50 & 0.56 & 0.56 & 0.01 \\
 & Q\&A & \cellcolor{cyan!13.1} 0.05 & \cellcolor{cyan!14.2} 0.25 & 0.57 & 0.56 & 0.56 & 0.02 \\
\multirow{2}{*}{Yi 34B (it)} & Num. & \cellcolor{cyan!4.1} 0.06 & \cellcolor{cyan!10.6} 0.25 & 0.50 & \cellcolor{orange!25.0} 0.44 & 0.56 & 0.00 \\
 & Q\&A & 0.35 & 0.36 & 0.65 & 0.56 & 0.60 & 0.02 \\
\multirow{2}{*}{Yi 34B} & Num. & 0.14 & 0.27 & 0.53 & \cellcolor{orange!25.0} 0.44 & 0.57 & 0.07 \\
 & Q\&A & 0.08 & \cellcolor{cyan!25.0} 0.24 & 0.62 & 0.56 & 0.54 & 0.06 \\
\multirow{2}{*}{Gemma 7B (it)} & Num. & 0.10 & \cellcolor{cyan!4.7} 0.26 & \cellcolor{orange!10.6} 0.49 & \cellcolor{orange!25.0} 0.44 & 0.56 & 0.01 \\
 & Q\&A & \cellcolor{orange!12.5} 0.42 & 0.43 & 0.53 & 0.56 & \cellcolor{orange!25.0} 0.50 & 0.02 \\
\multirow{2}{*}{Gemma 2B (it)} & Num. & 0.19 & 0.28 & \cellcolor{orange!0.7} 0.50 & 0.56 & 0.56 & 0.00 \\
 & Q\&A & 0.34 & 0.36 & \cellcolor{orange!6.2} 0.49 & 0.56 & 0.54 & 0.03 \\
\multirow{2}{*}{Gemma 7B} & Num. & \cellcolor{cyan!25.0} 0.03 & \cellcolor{cyan!13.0} 0.25 & 0.52 & 0.55 & 0.54 & 0.07 \\
 & Q\&A & \cellcolor{cyan!15.5} 0.04 & \cellcolor{cyan!19.0} 0.24 & 0.61 & 0.58 & 0.59 & 0.02 \\
\multirow{2}{*}{Gemma 2B} & Num. & \cellcolor{orange!20.2} 0.44 & \cellcolor{orange!14.2} 0.44 & \cellcolor{orange!0.7} 0.50 & 0.56 & 0.56 & 0.00 \\
 & Q\&A & 0.09 & \cellcolor{cyan!4.7} 0.26 & \cellcolor{orange!21.7} 0.48 & \cellcolor{orange!25.0} 0.44 & 0.54 & 0.01 \\
\midrule
LR & - & 0.04 & 0.24 & 0.58 & 0.56 & - & - \\
% GBM & - & 0.02 & 0.20 & 0.75 & 0.69 & - & - \\
XGBoost & - & 0.02 & 0.19 & 0.77 & 0.70 & - & - \\
\bottomrule
\end{tabular}


==> tables/both_prompting_schemes_different_rows/acstraveltime_sorted_by_size.tex <==
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\shortstack{Prompting\\ scheme}}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{ROC \\ AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
\multirow{2}{*}{GPT 4o mini (it)} & Num. & 0.15 & 0.27 & 0.58 & 0.57 & 0.51 & 0.22 \\
 & Q\&A & 0.39 & 0.40 & 0.65 & 0.55 & 0.60 & 0.36 \\
\multirow{2}{*}{Llama 3 70B (it)} & Num. & 0.12 & \cellcolor{cyan!21.4} 0.24 & 0.64 & 0.53 & \cellcolor{cyan!22.9} 0.61 & 0.13 \\
 & Q\&A & 0.15 & \cellcolor{cyan!22.6} 0.24 & \cellcolor{cyan!25.0} 0.70 & \cellcolor{cyan!25.0} 0.60 & \cellcolor{cyan!16.5} 0.61 & 0.12 \\
\multirow{2}{*}{Llama 3 70B} & Num. & 0.08 & \cellcolor{cyan!11.8} 0.25 & 0.52 & 0.46 & 0.56 & 0.05 \\
 & Q\&A & 0.09 & \cellcolor{cyan!21.4} 0.24 & 0.67 & 0.55 & \cellcolor{cyan!16.5} 0.61 & 0.05 \\
\multirow{2}{*}{Mixtral 8x22B (it)} & Num. & 0.12 & \cellcolor{cyan!22.6} 0.24 & 0.64 & \cellcolor{cyan!20.3} 0.59 & \cellcolor{cyan!25.0} 0.61 & 0.14 \\
 & Q\&A & 0.31 & 0.33 & 0.66 & \cellcolor{cyan!17.1} 0.59 & \cellcolor{cyan!8.1} 0.61 & 0.15 \\
\multirow{2}{*}{Mistral 8x22B} & Num. & 0.30 & 0.34 & 0.57 & 0.58 & 0.58 & 0.17 \\
 & Q\&A & 0.20 & 0.28 & 0.63 & \cellcolor{orange!25.0} 0.44 & 0.56 & 0.04 \\
\multirow{2}{*}{Yi 34B (it)} & Num. & \cellcolor{cyan!4.1} 0.06 & \cellcolor{cyan!10.6} 0.25 & 0.50 & \cellcolor{orange!25.0} 0.44 & 0.56 & 0.00 \\
 & Q\&A & 0.35 & 0.36 & 0.65 & 0.56 & 0.60 & 0.02 \\
\multirow{2}{*}{Yi 34B} & Num. & 0.14 & 0.27 & 0.53 & \cellcolor{orange!25.0} 0.44 & 0.57 & 0.07 \\
 & Q\&A & 0.08 & \cellcolor{cyan!25.0} 0.24 & 0.62 & 0.56 & 0.54 & 0.06 \\
\multirow{2}{*}{Mixtral 8x7B (it)} & Num. & 0.09 & \cellcolor{cyan!23.8} 0.24 & 0.61 & 0.57 & \cellcolor{orange!18.6} 0.50 & 0.11 \\
 & Q\&A & \cellcolor{orange!25.0} 0.45 & \cellcolor{orange!25.0} 0.45 & 0.66 & 0.52 & 0.55 & 0.29 \\
\multirow{2}{*}{Mistral 8x7B} & Num. & 0.07 & \cellcolor{cyan!15.4} 0.25 & 0.57 & 0.58 & 0.57 & 0.12 \\
 & Q\&A & 0.28 & 0.32 & 0.60 & \cellcolor{orange!25.0} 0.44 & 0.52 & 0.03 \\
\multirow{2}{*}{Llama 3 8B (it)} & Num. & 0.11 & \cellcolor{cyan!11.8} 0.25 & 0.56 & 0.56 & 0.52 & 0.06 \\
 & Q\&A & 0.19 & 0.28 & 0.60 & 0.57 & 0.57 & 0.11 \\
\multirow{2}{*}{Llama 3 8B} & Num. & 0.12 & 0.26 & \cellcolor{orange!25.0} 0.48 & \cellcolor{orange!25.0} 0.44 & 0.55 & 0.02 \\
 & Q\&A & 0.08 & \cellcolor{cyan!7.1} 0.25 & 0.53 & 0.56 & 0.52 & 0.03 \\
\multirow{2}{*}{Mistral 7B (it)} & Num. & 0.11 & \cellcolor{cyan!10.6} 0.25 & 0.55 & 0.56 & \cellcolor{orange!18.6} 0.50 & 0.10 \\
 & Q\&A & \cellcolor{orange!3.5} 0.41 & 0.42 & 0.59 & 0.57 & 0.53 & 0.19 \\
\multirow{2}{*}{Mistral 7B} & Num. & \cellcolor{orange!20.2} 0.44 & \cellcolor{orange!14.2} 0.44 & \cellcolor{orange!0.7} 0.50 & 0.56 & 0.56 & 0.01 \\
 & Q\&A & \cellcolor{cyan!13.1} 0.05 & \cellcolor{cyan!14.2} 0.25 & 0.57 & 0.56 & 0.56 & 0.02 \\
\multirow{2}{*}{Gemma 7B (it)} & Num. & 0.10 & \cellcolor{cyan!4.7} 0.26 & \cellcolor{orange!10.6} 0.49 & \cellcolor{orange!25.0} 0.44 & 0.56 & 0.01 \\
 & Q\&A & \cellcolor{orange!12.5} 0.42 & 0.43 & 0.53 & 0.56 & \cellcolor{orange!25.0} 0.50 & 0.02 \\
\multirow{2}{*}{Gemma 2B (it)} & Num. & 0.19 & 0.28 & \cellcolor{orange!0.7} 0.50 & 0.56 & 0.56 & 0.00 \\
 & Q\&A & 0.34 & 0.36 & \cellcolor{orange!6.2} 0.49 & 0.56 & 0.54 & 0.03 \\
\multirow{2}{*}{Gemma 7B} & Num. & \cellcolor{cyan!25.0} 0.03 & \cellcolor{cyan!13.0} 0.25 & 0.52 & 0.55 & 0.54 & 0.07 \\
 & Q\&A & \cellcolor{cyan!15.5} 0.04 & \cellcolor{cyan!19.0} 0.24 & 0.61 & 0.58 & 0.59 & 0.02 \\
\multirow{2}{*}{Gemma 2B} & Num. & \cellcolor{orange!20.2} 0.44 & \cellcolor{orange!14.2} 0.44 & \cellcolor{orange!0.7} 0.50 & 0.56 & 0.56 & 0.00 \\
 & Q\&A & 0.09 & \cellcolor{cyan!4.7} 0.26 & \cellcolor{orange!21.7} 0.48 & \cellcolor{orange!25.0} 0.44 & 0.54 & 0.01 \\
\midrule
LR & - & 0.04 & 0.24 & 0.58 & 0.56 & - & - \\
% GBM & - & 0.02 & 0.20 & 0.75 & 0.69 & - & - \\
XGBoost & - & 0.02 & 0.19 & 0.77 & 0.70 & - & - \\
\bottomrule
\end{tabular}


==> tables/multiple_choice_prompting/acsemployment.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
GPT 4o mini (it) & 0.28 & 0.29 & 0.79 & 0.65 & 0.74 & 0.41 \\
Llama 3 70B (it) & 0.17 & \cellcolor{cyan!17.1} 0.19 & \cellcolor{cyan!23.3} 0.85 & \cellcolor{cyan!15.4} 0.73 & \cellcolor{cyan!25.0} 0.78 & 0.29 \\
Llama 3 70B & 0.25 & 0.26 & \cellcolor{cyan!2.3} 0.82 & 0.52 & 0.74 & 0.12 \\
Llama 3 8B (it) & 0.07 & \cellcolor{cyan!25.0} 0.19 & 0.79 & \cellcolor{cyan!25.0} 0.74 & 0.74 & 0.22 \\
Llama 3 8B & 0.34 & 0.34 & 0.76 & \cellcolor{orange!25.0} 0.45 & 0.69 & 0.06 \\
Mixtral 8x22B (it) & \cellcolor{orange!23.0} 0.38 & \cellcolor{orange!8.0} 0.39 & 0.60 & 0.51 & 0.60 & 0.26 \\
Mixtral 8x22B & 0.21 & 0.24 & \cellcolor{cyan!25.0} 0.86 & 0.52 & \cellcolor{cyan!20.0} 0.78 & 0.08 \\
Mixtral 8x7B (it) & 0.22 & 0.24 & \cellcolor{cyan!6.8} 0.82 & \cellcolor{cyan!13.7} 0.73 & 0.75 & 0.44 \\
Mixtral 8x7B & 0.30 & 0.31 & \cellcolor{cyan!1.1} 0.81 & \cellcolor{orange!24.1} 0.45 & 0.74 & 0.06 \\
Mistral 7B (it) & \cellcolor{orange!6.6} 0.35 & 0.36 & 0.72 & 0.63 & 0.66 & 0.49 \\
Mistral 7B & 0.26 & 0.30 & 0.76 & \cellcolor{orange!25.0} 0.45 & 0.69 & 0.04 \\
Yi 34B (it) & 0.14 & 0.21 & 0.79 & 0.69 & 0.73 & 0.20 \\
Yi 34B & 0.08 & 0.23 & 0.70 & 0.62 & 0.64 & 0.12 \\
Gemma 7B (it) & \cellcolor{orange!10.0} 0.36 & 0.38 & 0.59 & 0.58 & 0.59 & 0.44 \\
Gemma 2B (it) & \cellcolor{orange!25.0} 0.38 & \cellcolor{orange!25.0} 0.41 & \cellcolor{orange!25.0} 0.42 & \cellcolor{orange!16.3} 0.46 & \cellcolor{orange!25.0} 0.48 & 0.23 \\
Gemma 7B & 0.15 & 0.25 & 0.65 & \cellcolor{orange!4.1} 0.48 & 0.63 & 0.13 \\
Gemma 2B & \cellcolor{cyan!25.0} 0.01 & 0.24 & 0.63 & 0.54 & 0.61 & 0.03 \\
\midrule
LR &  0.02 & 0.15 & 0.86 & 0.78 & - & - \\
% GBM & 0.00 & 0.12 & 0.91 & 0.83 & - & - \\
XGBoost  & 0.00 & 0.12 & 0.91 & 0.83 & - & - \\
\bottomrule
\end{tabular}


==> tables/multiple_choice_prompting/acsincome.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
GPT 4o mini (it) & 0.24 & 0.24 & \cellcolor{cyan!17.6} 0.85 & 0.74 & \cellcolor{cyan!21.1} 0.78 & 0.48 \\
Llama 3 70B (it) & 0.27 & 0.27 & \cellcolor{cyan!25.0} 0.86 & 0.69 & \cellcolor{cyan!14.5} 0.78 & 0.42 \\
Llama 3 70B & 0.20 & \cellcolor{cyan!14.9} 0.20 & \cellcolor{cyan!20.8} 0.86 & 0.70 & \cellcolor{cyan!25.0} 0.78 & 0.14 \\
Llama 3 8B (it) & 0.32 & 0.30 & \cellcolor{cyan!13.3} 0.85 & 0.62 & 0.73 & 0.37 \\
Llama 3 8B & 0.25 & 0.26 & 0.81 & \cellcolor{orange!20.8} 0.38 & 0.70 & 0.05 \\
Mixtral 8x22B (it) & 0.21 & \cellcolor{cyan!3.6} 0.22 & \cellcolor{cyan!11.2} 0.85 & \cellcolor{cyan!11.1} 0.76 & 0.75 & 0.48 \\
Mixtral 8x22B & \cellcolor{cyan!13.2} 0.17 & \cellcolor{cyan!21.6} 0.19 & \cellcolor{cyan!16.5} 0.85 & 0.68 & 0.74 & 0.10 \\
Mixtral 8x7B (it) & \cellcolor{cyan!16.8} 0.16 & \cellcolor{cyan!25.0} 0.18 & \cellcolor{cyan!19.7} 0.86 & \cellcolor{cyan!25.0} 0.78 & \cellcolor{cyan!21.1} 0.78 & 0.42 \\
Mixtral 8x7B & \cellcolor{cyan!10.6} 0.17 & \cellcolor{cyan!11.5} 0.21 & 0.83 & 0.65 & 0.76 & 0.06 \\
Mistral 7B (it) & 0.21 & \cellcolor{cyan!4.7} 0.22 & 0.83 & \cellcolor{cyan!16.5} 0.77 & \cellcolor{cyan!1.3} 0.77 & 0.42 \\
Mistral 7B & 0.20 & 0.23 & 0.80 & 0.73 & 0.74 & 0.04 \\
Yi 34B (it) & \cellcolor{cyan!1.3} 0.19 & \cellcolor{cyan!18.8} 0.19 & \cellcolor{cyan!19.7} 0.86 & 0.72 & 0.74 & 0.34 \\
Yi 34B & 0.25 & \cellcolor{cyan!2.5} 0.22 & \cellcolor{cyan!13.3} 0.85 & 0.62 & \cellcolor{cyan!3.9} 0.77 & 0.20 \\
Gemma 7B (it) & \cellcolor{orange!14.7} 0.61 & \cellcolor{orange!4.7} 0.59 & \cellcolor{cyan!3.8} 0.84 & \cellcolor{orange!25.0} 0.37 & 0.70 & 0.06 \\
Gemma 2B (it) & \cellcolor{orange!25.0} 0.63 & \cellcolor{orange!25.0} 0.63 & 0.73 & \cellcolor{orange!25.0} 0.37 & 0.63 & 0.00 \\
Gemma 7B & 0.24 & 0.27 & 0.76 & \cellcolor{orange!25.0} 0.37 & 0.69 & 0.04 \\
Gemma 2B & \cellcolor{cyan!25.0} 0.14 & 0.25 & \cellcolor{orange!25.0} 0.62 & 0.45 & \cellcolor{orange!25.0} 0.59 & 0.02 \\
\midrule
LR &  0.03 & 0.18 & 0.79 & 0.74 & - & - \\
% GBM &  0.01 & 0.13 & 0.89 & 0.81 & - & - \\
XGBoost  & 0.00 & 0.13 & 0.90 & 0.82 & - & - \\
\bottomrule
\end{tabular}


==> tables/multiple_choice_prompting/acsmobility.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
GPT 4o mini (it) & 0.26 & 0.26 & \cellcolor{cyan!0.6} 0.57 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!18.4} 0.67 & 0.02 \\
Llama 3 70B (it) & 0.20 & \cellcolor{cyan!1.5} 0.25 & 0.57 & 0.58 & 0.63 & 0.18 \\
Llama 3 70B & 0.22 & \cellcolor{cyan!4.8} 0.24 & 0.55 & 0.53 & 0.49 & 0.04 \\
Llama 3 8B (it) & 0.15 & \cellcolor{cyan!13.7} 0.22 & 0.56 & \cellcolor{cyan!5.3} 0.70 & 0.54 & 0.17 \\
Llama 3 8B & \cellcolor{cyan!12.5} 0.10 & \cellcolor{cyan!21.7} 0.20 & 0.55 & \cellcolor{cyan!24.5} 0.73 & 0.50 & 0.04 \\
Mixtral 8x22B (it) & 0.40 & 0.40 & \cellcolor{orange!12.8} 0.51 & 0.39 & 0.53 & 0.24 \\
Mixtral 8x22B & \cellcolor{cyan!10.2} 0.11 & \cellcolor{cyan!21.2} 0.21 & 0.55 & \cellcolor{cyan!25.0} 0.73 & 0.62 & 0.02 \\
Mixtral 8x7B (it) & 0.26 & 0.26 & \cellcolor{cyan!12.8} 0.58 & \cellcolor{cyan!25.0} 0.73 & 0.64 & 0.02 \\
Mixtral 8x7B & \cellcolor{cyan!0.8} 0.14 & \cellcolor{cyan!18.9} 0.21 & 0.57 & \cellcolor{cyan!25.0} 0.73 & 0.57 & 0.03 \\
Mistral 7B (it) & 0.26 & 0.26 & 0.57 & \cellcolor{cyan!25.0} 0.73 & 0.54 & 0.02 \\
Mistral 7B & 0.20 & \cellcolor{cyan!8.6} 0.23 & 0.53 & \cellcolor{cyan!23.4} 0.73 & \cellcolor{orange!25.0} 0.34 & 0.01 \\
Yi 34B (it) & \cellcolor{cyan!18.2} 0.09 & \cellcolor{cyan!23.1} 0.20 & 0.56 & \cellcolor{cyan!15.4} 0.72 & 0.59 & 0.15 \\
Yi 34B & \cellcolor{cyan!25.0} 0.07 & \cellcolor{cyan!25.0} 0.20 & 0.57 & \cellcolor{cyan!20.7} 0.73 & \cellcolor{cyan!11.1} 0.66 & 0.08 \\
Gemma 7B (it) & 0.25 & 0.26 & \cellcolor{cyan!25.0} 0.58 & \cellcolor{cyan!21.8} 0.73 & \cellcolor{cyan!25.0} 0.68 & 0.11 \\
Gemma 2B (it) & \cellcolor{orange!25.0} 0.73 & \cellcolor{orange!25.0} 0.73 & 0.52 & \cellcolor{orange!25.0} 0.27 & 0.40 & 0.00 \\
Gemma 7B & 0.41 & 0.37 & \cellcolor{orange!25.0} 0.50 & \cellcolor{orange!25.0} 0.27 & 0.41 & 0.10 \\
Gemma 2B & 0.25 & 0.26 & 0.51 & 0.34 & 0.48 & 0.02 \\
\midrule
LR &  0.02 & 0.19 & 0.61 & 0.74 & - & - \\
% GBM & 0.01 & 0.17 & 0.74 & 0.76 & - & - \\
XGBoost & 0.00 & 0.16 & 0.74 & 0.76 & - & - \\
\bottomrule
\end{tabular}

==> tables/multiple_choice_prompting/acspubliccoverage.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
GPT 4o mini (it) & 0.33 & 0.34 & \cellcolor{cyan!25.0} 0.71 & 0.60 & \cellcolor{cyan!9.6} 0.71 & 0.43 \\
Llama 3 70B (it) & 0.16 & \cellcolor{cyan!16.2} 0.21 & \cellcolor{cyan!7.0} 0.69 & \cellcolor{cyan!25.0} 0.75 & 0.52 & 0.20 \\
Llama 3 70B & 0.18 & \cellcolor{cyan!8.3} 0.22 & 0.67 & 0.63 & \cellcolor{cyan!25.0} 0.74 & 0.07 \\
Llama 3 8B (it) & 0.11 & \cellcolor{cyan!12.7} 0.21 & 0.59 & \cellcolor{cyan!7.7} 0.71 & \cellcolor{cyan!5.5} 0.71 & 0.19 \\
Llama 3 8B & 0.41 & 0.38 & 0.55 & \cellcolor{orange!25.0} 0.30 & 0.50 & 0.02 \\
Mixtral 8x22B (it) & 0.24 & 0.25 & \cellcolor{cyan!11.7} 0.70 & \cellcolor{cyan!12.7} 0.72 & 0.69 & 0.17 \\
Mixtral 8x22B & 0.32 & 0.30 & 0.59 & \cellcolor{orange!25.0} 0.30 & 0.56 & 0.05 \\
Mixtral 8x7B (it) & 0.20 & \cellcolor{cyan!7.4} 0.23 & \cellcolor{cyan!12.7} 0.70 & \cellcolor{cyan!23.3} 0.74 & \cellcolor{cyan!14.4} 0.72 & 0.35 \\
Mixtral 8x7B & 0.41 & 0.37 & 0.57 & \cellcolor{orange!25.0} 0.30 & 0.38 & 0.03 \\
Mistral 7B (it) & 0.30 & 0.30 & 0.61 & \cellcolor{cyan!0.4} 0.70 & 0.68 & 0.01 \\
Mistral 7B & 0.29 & 0.30 & \cellcolor{orange!25.0} 0.45 & \cellcolor{orange!25.0} 0.30 & \cellcolor{cyan!2.0} 0.70 & 0.02 \\
Yi 34B (it) & \cellcolor{cyan!16.7} 0.06 & \cellcolor{cyan!25.0} 0.19 & 0.67 & \cellcolor{cyan!19.4} 0.74 & 0.70 & 0.13 \\
Yi 34B & \cellcolor{cyan!25.0} 0.04 & \cellcolor{cyan!17.2} 0.21 & 0.59 & \cellcolor{cyan!2.1} 0.70 & 0.56 & 0.07 \\
Gemma 7B (it) & 0.30 & 0.34 & \cellcolor{orange!14.6} 0.46 & 0.50 & \cellcolor{orange!25.0} 0.32 & 0.32 \\
Gemma 2B (it) & \cellcolor{orange!25.0} 0.70 & \cellcolor{orange!25.0} 0.70 & 0.54 & \cellcolor{orange!25.0} 0.30 & \cellcolor{orange!17.9} 0.33 & 0.00 \\
Gemma 7B & 0.15 & \cellcolor{cyan!3.4} 0.23 & 0.49 & 0.49 & 0.37 & 0.10 \\
Gemma 2B & 0.26 & 0.28 & 0.54 & \cellcolor{orange!25.0} 0.30 & 0.62 & 0.01 \\
\midrule
LR & 0.03 & 0.19 & 0.70 & 0.72 & - & - \\
% GBM & 0.01 & 0.14 & 0.83 & 0.80 & - & - \\
XGBoost & 0.00 & 0.14 & 0.84 & 0.80 & - & - \\
\bottomrule
\end{tabular}



==> tables/multiple_choice_prompting/acstraveltime.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
GPT 4o mini (it) & 0.39 & 0.40 & 0.65 & 0.55 & \cellcolor{cyan!7.5} 0.60 & 0.36 \\
Llama 3 70B (it) & 0.15 & \cellcolor{cyan!22.6} 0.24 & \cellcolor{cyan!25.0} 0.70 & \cellcolor{cyan!25.0} 0.60 & \cellcolor{cyan!25.0} 0.61 & 0.12 \\
Llama 3 70B & 0.09 & \cellcolor{cyan!21.4} 0.24 & 0.67 & 0.55 & \cellcolor{cyan!25.0} 0.61 & 0.05 \\
Llama 3 8B (it) & 0.19 & 0.28 & 0.60 & 0.57 & 0.57 & 0.11 \\
Llama 3 8B & 0.08 & \cellcolor{cyan!7.1} 0.25 & 0.53 & 0.56 & 0.52 & 0.03 \\
Mixtral 8x22B (it) & 0.31 & 0.33 & 0.66 & \cellcolor{cyan!17.1} 0.59 & \cellcolor{cyan!16.2} 0.61 & 0.15 \\
Mixtral 8x22B & 0.20 & 0.28 & 0.63 & \cellcolor{orange!25.0} 0.44 & 0.56 & 0.04 \\
Mixtral 8x7B (it) & \cellcolor{orange!25.0} 0.45 & \cellcolor{orange!25.0} 0.45 & 0.66 & 0.52 & 0.55 & 0.29 \\
Mixtral 8x7B & 0.28 & 0.32 & 0.60 & \cellcolor{orange!25.0} 0.44 & 0.52 & 0.03 \\
Mistral 7B (it) & \cellcolor{orange!2.7} 0.41 & 0.42 & 0.59 & 0.57 & 0.53 & 0.19 \\
Mistral 7B & \cellcolor{cyan!22.5} 0.05 & \cellcolor{cyan!14.2} 0.25 & 0.57 & 0.56 & 0.56 & 0.02 \\
Yi 34B (it) & 0.35 & 0.36 & 0.65 & 0.56 & \cellcolor{cyan!3.1} 0.60 & 0.02 \\
Yi 34B & \cellcolor{cyan!4.5} 0.08 & \cellcolor{cyan!25.0} 0.24 & 0.62 & 0.56 & 0.54 & 0.06 \\
Gemma 7B (it) & \cellcolor{orange!12.0} 0.42 & 0.43 & 0.53 & 0.56 & \cellcolor{orange!25.0} 0.50 & 0.02 \\
Gemma 2B (it) & 0.34 & 0.36 & \cellcolor{orange!9.3} 0.49 & 0.56 & 0.54 & 0.03 \\
Gemma 7B & \cellcolor{cyan!25.0} 0.04 & \cellcolor{cyan!19.0} 0.24 & 0.61 & 0.58 & 0.59 & 0.02 \\
Gemma 2B & 0.09 & \cellcolor{cyan!4.7} 0.26 & \cellcolor{orange!25.0} 0.48 & \cellcolor{orange!25.0} 0.44 & 0.54 & 0.01 \\
\midrule
LR & 0.04 & 0.24 & 0.58 & 0.56 & - & - \\
% GBM & 0.02 & 0.20 & 0.75 & 0.69 & - & - \\
XGBoost & 0.02 & 0.19 & 0.77 & 0.70 & - & - \\
\bottomrule
\end{tabular}

==> tables/multiple_choice_prompting/legacy/acsemployment-colored.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^*$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
Llama 3 70B (it) & 0.17 & \cellcolor{cyan!18.2} 0.19 & \cellcolor{cyan!22.7} 0.85 & \cellcolor{cyan!16.3} 0.73 & \cellcolor{cyan!25.0} 0.78 & 0.29 \\
Llama 3 70B & 0.25 & 0.26 & \cellcolor{cyan!1.2} 0.82 & 0.51 & 0.74 & 0.12 \\
Llama 3 8B (it) & 0.07 & \cellcolor{cyan!25.0} 0.19 & 0.79 & \cellcolor{cyan!25.0} 0.74 & 0.74 & 0.22 \\
Llama 3 8B & 0.34 & 0.34 & 0.75 & \cellcolor{orange!25.0} 0.45 & 0.68 & 0.06 \\
Mixtral 8x22B (it) & \cellcolor{orange!24.3} 0.38 & \cellcolor{orange!9.2} 0.39 & 0.60 & 0.51 & 0.60 & 0.26 \\
Mixtral 8x22B & 0.21 & 0.24 & \cellcolor{cyan!25.0} 0.86 & 0.52 & \cellcolor{cyan!16.7} 0.77 & 0.08 \\
Mixtral 8x7B (it) & 0.22 & 0.23 & \cellcolor{cyan!6.9} 0.83 & \cellcolor{cyan!16.3} 0.73 & \cellcolor{cyan!0.2} 0.75 & 0.44 \\
Mixtral 8x7B & 0.29 & 0.31 & \cellcolor{cyan!0.1} 0.81 & \cellcolor{orange!24.1} 0.45 & 0.74 & 0.06 \\
Mistral 7B (it) & \cellcolor{orange!6.6} 0.35 & 0.36 & 0.72 & 0.63 & 0.66 & 0.49 \\
Mistral 7B & 0.26 & 0.30 & 0.76 & \cellcolor{orange!25.0} 0.45 & 0.69 & 0.04 \\
Yi 34B (chat) & 0.14 & 0.21 & 0.79 & 0.69 & 0.73 & 0.20 \\
Yi 34B & 0.08 & 0.23 & 0.70 & 0.62 & 0.63 & 0.11 \\
Gemma 7B (it) & \cellcolor{orange!10.0} 0.36 & 0.38 & 0.59 & 0.58 & 0.59 & 0.44 \\
Gemma 7B & 0.16 & 0.25 & 0.65 & \cellcolor{orange!4.1} 0.48 & 0.64 & 0.13 \\
Gemma 2B (it) & \cellcolor{orange!25.0} 0.38 & \cellcolor{orange!25.0} 0.41 & \cellcolor{orange!25.0} 0.42 & \cellcolor{orange!16.3} 0.46 & \cellcolor{orange!25.0} 0.48 & 0.23 \\
Gemma 2B & \cellcolor{cyan!25.0} 0.01 & 0.24 & 0.63 & 0.54 & 0.61 & 0.03 \\
\midrule
LR & 0.02 & 0.15 & 0.86 & 0.78 & - & - \\
% GBM & 0.00 & 0.12 & 0.91 & 0.83 & - & - \\
XGBoost & 0.00 & 0.12 & 0.91 & 0.83 & - & - \\
\bottomrule
\end{tabular}

==> tables/multiple_choice_prompting/legacy/acsincome-colored.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^*$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
GPT 4o mini (it) & 0.24 & 0.24 & \cellcolor{cyan!21.5} 0.85 & 0.74 & 0.75 & 0.48 \\
Llama 3 70B (it) & 0.27 & 0.27 & \cellcolor{cyan!25.0} 0.86 & 0.69 & \cellcolor{cyan!15.3} 0.78 & 0.42 \\
Llama 3 70B & 0.20 & \cellcolor{cyan!14.9} 0.20 & \cellcolor{cyan!20.8} 0.86 & 0.70 & \cellcolor{cyan!10.5} 0.77 & 0.14 \\
Llama 3 8B (it) & 0.32 & 0.30 & \cellcolor{cyan!13.3} 0.85 & 0.62 & \cellcolor{cyan!15.3} 0.78 & 0.37 \\
Llama 3 8B & 0.25 & 0.26 & 0.81 & \cellcolor{orange!20.2} 0.38 & 0.69 & 0.05 \\
Mixtral 8x22B (it) & 0.21 & \cellcolor{cyan!3.6} 0.22 & \cellcolor{cyan!11.2} 0.85 & \cellcolor{cyan!11.1} 0.76 & 0.75 & 0.48 \\
Mixtral 8x22B & \cellcolor{cyan!13.7} 0.17 & \cellcolor{cyan!22.2} 0.19 & \cellcolor{cyan!16.5} 0.85 & 0.68 & \cellcolor{cyan!7.3} 0.77 & 0.10 \\
Mixtral 8x7B (it) & \cellcolor{cyan!17.3} 0.16 & \cellcolor{cyan!25.0} 0.18 & \cellcolor{cyan!19.7} 0.86 & \cellcolor{cyan!25.0} 0.78 & \cellcolor{cyan!25.0} 0.78 & 0.42 \\
Mixtral 8x7B & \cellcolor{cyan!10.6} 0.17 & \cellcolor{cyan!11.5} 0.21 & 0.83 & 0.65 & 0.74 & 0.06 \\
Mistral 7B (it) & 0.21 & \cellcolor{cyan!4.7} 0.22 & 0.83 & \cellcolor{cyan!16.5} 0.77 & \cellcolor{cyan!0.8} 0.77 & 0.42 \\
Mistral 7B & 0.20 & 0.23 & 0.80 & 0.73 & 0.74 & 0.04 \\
Yi 34B (chat) & \cellcolor{cyan!1.8} 0.19 & \cellcolor{cyan!18.8} 0.19 & \cellcolor{cyan!19.7} 0.86 & 0.72 & 0.74 & 0.34 \\
Yi 34B & 0.24 & \cellcolor{cyan!2.5} 0.22 & \cellcolor{cyan!13.3} 0.85 & 0.62 & 0.74 & 0.20 \\
Gemma 7B (it) & \cellcolor{orange!14.7} 0.61 & \cellcolor{orange!4.2} 0.59 & \cellcolor{cyan!3.8} 0.84 & \cellcolor{orange!25.0} 0.37 & 0.75 & 0.06 \\
Gemma 7B & 0.24 & 0.27 & 0.76 & \cellcolor{orange!25.0} 0.37 & 0.68 & 0.04 \\
Gemma 2B (it) & \cellcolor{orange!25.0} 0.63 & \cellcolor{orange!25.0} 0.63 & 0.73 & \cellcolor{orange!25.0} 0.37 & \cellcolor{orange!20.2} 0.63 & 0.00 \\
Gemma 2B & \cellcolor{cyan!25.0} 0.14 & 0.25 & \cellcolor{orange!25.0} 0.62 & 0.45 & \cellcolor{orange!25.0} 0.63 & 0.02 \\
\midrule
LR & 0.03 & 0.18 & 0.79 & 0.74 & - & - \\
% GBM & 0.01 & 0.13 & 0.89 & 0.81 & - & - \\
XGBoost & 0.00 & 0.13 & 0.90 & 0.82 & - & - \\
\bottomrule
\end{tabular}


==> tables/multiple_choice_prompting/legacy/acsmobility-colored.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^*$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
Llama 3 70B (it) & 0.20 & \cellcolor{cyan!1.0} 0.25 & 0.57 & 0.61 & 0.48 & 0.18 \\
Llama 3 70B & 0.22 & \cellcolor{cyan!4.8} 0.24 & 0.55 & 0.67 & 0.53 & 0.04 \\
Llama 3 8B (it) & 0.15 & \cellcolor{cyan!13.7} 0.22 & 0.56 & \cellcolor{cyan!8.0} 0.70 & 0.53 & 0.17 \\
Llama 3 8B & \cellcolor{cyan!12.5} 0.10 & \cellcolor{cyan!22.2} 0.20 & 0.55 & \cellcolor{cyan!25.0} 0.73 & 0.63 & 0.04 \\
Mixtral 8x22B (it) & 0.41 & 0.40 & \cellcolor{orange!9.8} 0.51 & 0.40 & 0.50 & 0.24 \\
Mixtral 8x22B & \cellcolor{cyan!10.6} 0.11 & \cellcolor{cyan!21.7} 0.20 & 0.55 & \cellcolor{cyan!25.0} 0.73 & 0.63 & 0.02 \\
Mixtral 8x7B (it) & 0.26 & 0.26 & \cellcolor{cyan!9.8} 0.58 & \cellcolor{cyan!25.0} 0.73 & 0.60 & 0.02 \\
Mixtral 8x7B & \cellcolor{cyan!0.8} 0.14 & \cellcolor{cyan!18.9} 0.21 & 0.57 & \cellcolor{cyan!25.0} 0.73 & 0.52 & 0.03 \\
Mistral 7B (it) & 0.26 & 0.26 & 0.57 & \cellcolor{cyan!25.0} 0.73 & 0.54 & 0.02 \\
Mistral 7B & 0.20 & \cellcolor{cyan!8.6} 0.23 & 0.53 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{orange!25.0} 0.33 & 0.01 \\
Yi 34B (chat) & \cellcolor{cyan!18.2} 0.09 & \cellcolor{cyan!23.1} 0.20 & 0.56 & \cellcolor{cyan!18.1} 0.72 & 0.59 & 0.15 \\
Yi 34B & \cellcolor{cyan!25.0} 0.07 & \cellcolor{cyan!25.0} 0.20 & 0.57 & \cellcolor{cyan!23.9} 0.73 & 0.63 & 0.08 \\
Gemma 7B (it) & 0.25 & 0.26 & \cellcolor{cyan!25.0} 0.58 & \cellcolor{cyan!23.9} 0.73 & \cellcolor{cyan!25.0} 0.67 & 0.11 \\
Gemma 7B & 0.41 & 0.37 & \cellcolor{orange!25.0} 0.50 & 0.39 & 0.41 & 0.10 \\
Gemma 2B (it) & \cellcolor{orange!25.0} 0.73 & \cellcolor{orange!25.0} 0.73 & 0.52 & \cellcolor{orange!25.0} 0.27 & 0.40 & 0.00 \\
Gemma 2B & 0.25 & 0.26 & \cellcolor{orange!3.7} 0.51 & 0.39 & 0.45 & 0.02 \\
\midrule
LR & 0.02 & 0.19 & 0.61 & 0.74 & - & - \\
% GBM & 0.01 & 0.17 & 0.74 & 0.76 & - & - \\
XGBoost & 0.00 & 0.16 & 0.74 & 0.76 & - & - \\
\bottomrule
\end{tabular}

==> tables/multiple_choice_prompting/legacy/acspubliccoverage-colored.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^*$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
Llama 3 70B (it) & 0.16 & \cellcolor{cyan!16.2} 0.21 & \cellcolor{cyan!19.0} 0.69 & \cellcolor{cyan!25.0} 0.75 & 0.49 & 0.20 \\
Llama 3 70B & 0.18 & \cellcolor{cyan!8.3} 0.22 & 0.67 & 0.63 & 0.50 & 0.07 \\
Llama 3 8B (it) & 0.11 & \cellcolor{cyan!12.7} 0.21 & 0.59 & \cellcolor{cyan!7.7} 0.71 & \cellcolor{cyan!15.7} 0.71 & 0.19 \\
Llama 3 8B & 0.41 & 0.38 & 0.55 & \cellcolor{orange!25.0} 0.30 & 0.50 & 0.02 \\
Mixtral 8x22B (it) & 0.24 & 0.25 & \cellcolor{cyan!25.0} 0.70 & \cellcolor{cyan!12.2} 0.72 & 0.67 & 0.17 \\
Mixtral 8x22B & 0.32 & 0.30 & 0.59 & \cellcolor{orange!25.0} 0.30 & 0.56 & 0.05 \\
Mixtral 8x7B (it) & 0.20 & \cellcolor{cyan!7.4} 0.23 & \cellcolor{cyan!25.0} 0.70 & \cellcolor{cyan!23.3} 0.74 & \cellcolor{cyan!25.0} 0.72 & 0.35 \\
Mixtral 8x7B & 0.41 & 0.37 & 0.57 & \cellcolor{orange!25.0} 0.30 & 0.38 & 0.03 \\
Mistral 7B (it) & 0.30 & 0.30 & 0.61 & \cellcolor{cyan!0.4} 0.70 & 0.68 & 0.01 \\
Mistral 7B & 0.29 & 0.30 & \cellcolor{orange!25.0} 0.45 & \cellcolor{orange!25.0} 0.30 & \cellcolor{cyan!12.0} 0.70 & 0.02 \\
Yi 34B (chat) & \cellcolor{cyan!16.7} 0.06 & \cellcolor{cyan!25.0} 0.19 & 0.67 & \cellcolor{cyan!19.4} 0.74 & 0.68 & 0.13 \\
Yi 34B & \cellcolor{cyan!25.0} 0.04 & \cellcolor{cyan!17.2} 0.21 & 0.59 & \cellcolor{cyan!2.1} 0.70 & 0.56 & 0.07 \\
Gemma 7B (it) & 0.30 & 0.34 & \cellcolor{orange!14.0} 0.46 & 0.50 & \cellcolor{orange!25.0} 0.32 & 0.32 \\
Gemma 7B & 0.15 & \cellcolor{cyan!3.4} 0.23 & 0.49 & 0.49 & 0.37 & 0.10 \\
Gemma 2B (it) & \cellcolor{orange!25.0} 0.70 & \cellcolor{orange!25.0} 0.70 & 0.54 & \cellcolor{orange!25.0} 0.30 & \cellcolor{orange!17.6} 0.33 & 0.00 \\
Gemma 2B & 0.26 & 0.28 & 0.54 & \cellcolor{orange!25.0} 0.30 & 0.62 & 0.01 \\
\midrule
LR & 0.03 & 0.19 & 0.70 & 0.73 & - & - \\
% GBM & 0.01 & 0.14 & 0.83 & 0.80 & - & - \\
XGBoost & 0.00 & 0.14 & 0.84 & 0.80 & - & - \\
\bottomrule
\end{tabular}

==> tables/multiple_choice_prompting/legacy/acstraveltime-colored.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^*$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
Llama 3 70B (it) & 0.15 & \cellcolor{cyan!22.6} 0.24 & \cellcolor{cyan!25.0} 0.70 & \cellcolor{cyan!25.0} 0.60 & \cellcolor{cyan!25.0} 0.61 & 0.12 \\
Llama 3 70B & 0.09 & \cellcolor{cyan!22.6} 0.24 & 0.67 & 0.55 & \cellcolor{cyan!25.0} 0.61 & 0.05 \\
Llama 3 8B (it) & 0.19 & 0.28 & 0.60 & 0.57 & 0.57 & 0.11 \\
Llama 3 8B & 0.08 & \cellcolor{cyan!8.2} 0.25 & 0.53 & 0.56 & 0.54 & 0.03 \\
Mixtral 8x22B (it) & 0.32 & 0.33 & 0.66 & \cellcolor{cyan!17.1} 0.59 & \cellcolor{cyan!14.3} 0.61 & 0.15 \\
Mixtral 8x22B & 0.20 & 0.28 & 0.63 & \cellcolor{orange!25.0} 0.44 & 0.54 & 0.04 \\
Mixtral 8x7B (it) & \cellcolor{orange!25.0} 0.45 & \cellcolor{orange!25.0} 0.45 & 0.66 & 0.52 & 0.55 & 0.29 \\
Mixtral 8x7B & 0.28 & 0.32 & 0.60 & \cellcolor{orange!25.0} 0.44 & 0.56 & 0.03 \\
Mistral 7B (it) & \cellcolor{orange!2.7} 0.41 & 0.42 & 0.59 & 0.57 & 0.53 & 0.19 \\
Mistral 7B & \cellcolor{cyan!22.5} 0.05 & \cellcolor{cyan!16.6} 0.25 & 0.57 & 0.56 & 0.55 & 0.02 \\
Yi 34B (chat) & 0.35 & 0.36 & 0.65 & 0.56 & 0.52 & 0.02 \\
Yi 34B & \cellcolor{cyan!3.3} 0.08 & \cellcolor{cyan!25.0} 0.24 & 0.62 & 0.56 & 0.52 & 0.06 \\
Gemma 7B (it) & \cellcolor{orange!12.0} 0.42 & 0.43 & 0.53 & 0.56 & 0.50 & 0.02 \\
Gemma 7B & \cellcolor{cyan!25.0} 0.04 & \cellcolor{cyan!20.2} 0.24 & 0.61 & 0.58 & 0.57 & 0.02 \\
Gemma 2B (it) & 0.34 & 0.36 & \cellcolor{orange!9.3} 0.49 & 0.56 & 0.54 & 0.03 \\
Gemma 2B & 0.09 & \cellcolor{cyan!5.8} 0.26 & \cellcolor{orange!25.0} 0.48 & \cellcolor{orange!25.0} 0.44 & \cellcolor{orange!25.0} 0.45 & 0.01 \\
\midrule
LR & 0.04 & 0.24 & 0.58 & 0.56 & - & - \\
% GBM & 0.02 & 0.20 & 0.75 & 0.69 & - & - \\
XGBoost & 0.02 & 0.19 & 0.77 & 0.70 & - & - \\
\bottomrule
\end{tabular}

==> tables/numeric_prompting/acsemployment.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
GPT 4o mini (it) & 0.23 & 0.23 & 0.80 & 0.73 & 0.77 & 0.28 \\
Llama 3 70B (it) & \cellcolor{cyan!0.7} 0.05 & \cellcolor{cyan!25.0} 0.14 & \cellcolor{cyan!25.0} 0.88 & \cellcolor{cyan!25.0} 0.81 & \cellcolor{cyan!25.0} 0.81 & 0.32 \\
Llama 3 70B & 0.05 & \cellcolor{cyan!16.7} 0.15 & \cellcolor{cyan!13.6} 0.86 & \cellcolor{cyan!5.8} 0.78 & \cellcolor{cyan!3.1} 0.78 & 0.31 \\
Llama 3 8B (it) & 0.08 & 0.17 & 0.82 & 0.77 & 0.77 & 0.29 \\
Llama 3 8B & 0.15 & 0.23 & 0.75 & \cellcolor{orange!25.0} 0.46 & 0.68 & 0.11 \\
Mixtral 8x22B (it) & 0.06 & \cellcolor{cyan!21.9} 0.14 & \cellcolor{cyan!24.4} 0.87 & \cellcolor{cyan!16.5} 0.79 & \cellcolor{cyan!20.9} 0.80 & 0.33 \\
Mixtral 8x22B & 0.15 & 0.18 & 0.82 & \cellcolor{cyan!20.7} 0.80 & \cellcolor{cyan!15.3} 0.79 & 0.35 \\
Mixtral 8x7B (it) & 0.07 & \cellcolor{cyan!16.7} 0.15 & \cellcolor{cyan!23.2} 0.87 & \cellcolor{cyan!7.2} 0.78 & \cellcolor{cyan!7.1} 0.78 & 0.27 \\
Mixtral 8x7B & 0.08 & 0.17 & 0.81 & 0.73 & 0.75 & 0.25 \\
Mistral 7B (it) & \cellcolor{cyan!7.4} 0.04 & 0.19 & 0.79 & 0.69 & 0.76 & 0.27 \\
Mistral 7B & 0.14 & 0.19 & 0.80 & \cellcolor{cyan!12.9} 0.79 & \cellcolor{cyan!11.2} 0.79 & 0.42 \\
Yi 34B (it) & 0.15 & 0.21 & 0.81 & 0.51 & \cellcolor{cyan!12.8} 0.79 & 0.18 \\
Yi 34B & 0.13 & 0.23 & 0.66 & 0.50 & 0.64 & 0.11 \\
Gemma 7B (it) & \cellcolor{cyan!8.8} 0.04 & 0.22 & 0.71 & 0.60 & 0.66 & 0.20 \\
Gemma 2B (it) & 0.12 & 0.27 & \cellcolor{orange!25.0} 0.46 & \cellcolor{orange!25.0} 0.46 & \cellcolor{orange!25.0} 0.50 & 0.05 \\
Gemma 7B & \cellcolor{orange!25.0} 0.35 & \cellcolor{orange!25.0} 0.38 & \cellcolor{orange!1.6} 0.50 & 0.51 & \cellcolor{orange!4.7} 0.52 & 0.22 \\
Gemma 2B & \cellcolor{cyan!25.0} 0.01 & 0.23 & 0.57 & 0.53 & \cellcolor{orange!24.2} 0.50 & 0.12 \\
\midrule
LR & 0.02 & 0.15 & 0.86 & 0.78 & - & - \\
% GBM & 0.00 & 0.12 & 0.91 & 0.83 & - & - \\
XGBoost & 0.00 & 0.12 & 0.91 & 0.83 & - & - \\
\bottomrule
\end{tabular}



==> tables/numeric_prompting/acsincome.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
GPT 4o mini (it) & \cellcolor{cyan!25.0} 0.05 & \cellcolor{cyan!25.0} 0.16 & \cellcolor{cyan!20.6} 0.83 & \cellcolor{cyan!24.4} 0.78 & \cellcolor{cyan!12.3} 0.78 & 0.32 \\
Llama 3 70B (it) & 0.25 & 0.23 & \cellcolor{cyan!22.1} 0.84 & 0.67 & 0.74 & 0.29 \\
Llama 3 70B & 0.27 & 0.24 & \cellcolor{cyan!6.7} 0.82 & 0.54 & \cellcolor{cyan!25.0} 0.79 & 0.25 \\
Llama 3 8B (it) & 0.23 & 0.23 & \cellcolor{cyan!0.1} 0.81 & 0.67 & 0.67 & 0.16 \\
Llama 3 8B & 0.14 & 0.24 & 0.63 & \cellcolor{orange!3.7} 0.40 & 0.65 & 0.07 \\
Mixtral 8x22B (it) & 0.11 & \cellcolor{cyan!15.5} 0.17 & \cellcolor{cyan!25.0} 0.84 & \cellcolor{cyan!18.9} 0.77 & \cellcolor{cyan!1.3} 0.77 & 0.30 \\
Mixtral 8x22B & 0.13 & \cellcolor{cyan!3.6} 0.18 & \cellcolor{cyan!9.6} 0.82 & \cellcolor{cyan!2.4} 0.74 & 0.77 & 0.38 \\
Mixtral 8x7B (it) & 0.10 & \cellcolor{cyan!15.5} 0.17 & \cellcolor{cyan!22.8} 0.84 & \cellcolor{cyan!12.8} 0.76 & 0.73 & 0.28 \\
Mixtral 8x7B & \cellcolor{cyan!4.0} 0.07 & \cellcolor{cyan!13.1} 0.17 & \cellcolor{cyan!3.7} 0.81 & \cellcolor{cyan!25.0} 0.78 & 0.74 & 0.28 \\
Mistral 7B (it) & 0.16 & 0.19 & \cellcolor{cyan!14.7} 0.83 & 0.70 & 0.76 & 0.20 \\
Mistral 7B & \cellcolor{orange!15.7} 0.36 & 0.32 & 0.75 & 0.49 & 0.70 & 0.35 \\
Yi 34B (it) & 0.22 & 0.21 & 0.80 & 0.48 & \cellcolor{cyan!6.0} 0.77 & 0.20 \\
Yi 34B & 0.15 & 0.19 & \cellcolor{cyan!17.7} 0.83 & 0.61 & 0.75 & 0.23 \\
Gemma 7B (it) & 0.33 & 0.30 & 0.78 & 0.42 & \cellcolor{orange!25.0} 0.63 & 0.14 \\
Gemma 2B (it) & 0.28 & 0.31 & \cellcolor{orange!25.0} 0.50 & \cellcolor{orange!25.0} 0.37 & \cellcolor{orange!17.1} 0.63 & 0.00 \\
Gemma 7B & 0.15 & 0.20 & 0.80 & 0.73 & 0.74 & 0.24 \\
Gemma 2B & \cellcolor{orange!25.0} 0.37 & \cellcolor{orange!25.0} 0.37 & \cellcolor{orange!25.0} 0.50 & 0.63 & \cellcolor{orange!17.1} 0.63 & 0.00 \\
\midrule
LR & 0.03 & 0.18 & 0.79 & 0.74 & - & - \\
% GBM & 0.01 & 0.13 & 0.89 & 0.81 & - & - \\
XGBoost & 0.00 & 0.13 & 0.90 & 0.82 & - & - \\
\bottomrule
\end{tabular}



==> tables/numeric_prompting/acsmobility.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
GPT 4o mini (it) & 0.22 & 0.25 & 0.49 & \cellcolor{cyan!25.0} 0.73 & 0.62 & 0.09 \\
Llama 3 70B (it) & 0.05 & \cellcolor{cyan!10.7} 0.20 & 0.52 & \cellcolor{cyan!25.0} 0.73 & 0.52 & 0.08 \\
Llama 3 70B & 0.06 & \cellcolor{cyan!7.1} 0.20 & 0.53 & \cellcolor{cyan!20.7} 0.73 & 0.48 & 0.08 \\
Llama 3 8B (it) & 0.11 & 0.21 & 0.49 & \cellcolor{cyan!23.4} 0.73 & 0.67 & 0.06 \\
Llama 3 8B & 0.14 & 0.21 & 0.51 & \cellcolor{cyan!19.1} 0.72 & 0.64 & 0.09 \\
Mixtral 8x22B (it) & 0.05 & \cellcolor{cyan!17.9} 0.20 & \cellcolor{cyan!25.0} 0.54 & \cellcolor{cyan!25.0} 0.73 & 0.47 & 0.05 \\
Mixtral 8x22B & 0.13 & 0.22 & 0.49 & \cellcolor{cyan!25.0} 0.73 & 0.40 & 0.09 \\
Mixtral 8x7B (it) & 0.11 & 0.21 & 0.51 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!22.8} 0.73 & 0.02 \\
Mixtral 8x7B & 0.24 & 0.25 & \cellcolor{orange!25.0} 0.48 & \cellcolor{cyan!25.0} 0.73 & 0.47 & 0.03 \\
Mistral 7B (it) & 0.17 & 0.23 & 0.49 & \cellcolor{cyan!24.5} 0.73 & \cellcolor{cyan!1.9} 0.69 & 0.07 \\
Mistral 7B & \cellcolor{orange!25.0} 0.27 & \cellcolor{orange!25.0} 0.27 & 0.50 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!25.0} 0.73 & 0.00 \\
Yi 34B (it) & 0.23 & 0.25 & 0.50 & \cellcolor{orange!25.0} 0.27 & \cellcolor{cyan!25.0} 0.73 & 0.00 \\
Yi 34B & 0.15 & 0.23 & 0.52 & 0.44 & 0.44 & 0.12 \\
Gemma 7B (it) & \cellcolor{orange!8.9} 0.25 & 0.26 & \cellcolor{orange!3.1} 0.49 & \cellcolor{cyan!22.3} 0.73 & \cellcolor{cyan!22.3} 0.73 & 0.08 \\
Gemma 2B (it) & \cellcolor{cyan!25.0} 0.02 & \cellcolor{cyan!25.0} 0.20 & 0.50 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{orange!25.0} 0.27 & 0.01 \\
Gemma 7B & 0.19 & 0.24 & 0.49 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!25.0} 0.73 & 0.06 \\
Gemma 2B & \cellcolor{orange!25.0} 0.27 & \cellcolor{orange!25.0} 0.27 & 0.50 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!25.0} 0.73 & 0.00 \\
\midrule
LR & 0.02 & 0.19 & 0.61 & 0.74 & - & - \\
% GBM & 0.01 & 0.17 & 0.74 & 0.76 & - & - \\
XGBoost & 0.00 & 0.16 & 0.74 & 0.76 & - & - \\
\bottomrule
\end{tabular}


==> tables/numeric_prompting/acspubliccoverage.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
GPT 4o mini (it) & 0.10 & 0.20 & 0.68 & \cellcolor{cyan!17.6} 0.73 & 0.61 & 0.26 \\
Llama 3 70B (it) & 0.13 & 0.20 & \cellcolor{cyan!25.0} 0.73 & \cellcolor{cyan!24.4} 0.75 & \cellcolor{cyan!25.0} 0.75 & 0.23 \\
Llama 3 70B & 0.12 & 0.21 & 0.64 & 0.53 & 0.51 & 0.20 \\
Llama 3 8B (it) & 0.17 & 0.22 & 0.64 & 0.68 & 0.69 & 0.09 \\
Llama 3 8B & 0.20 & 0.25 & 0.51 & \cellcolor{orange!6.2} 0.34 & \cellcolor{orange!25.0} 0.34 & 0.07 \\
Mixtral 8x22B (it) & \cellcolor{cyan!25.0} 0.04 & \cellcolor{cyan!25.0} 0.18 & \cellcolor{cyan!11.0} 0.71 & \cellcolor{cyan!25.0} 0.75 & 0.57 & 0.21 \\
Mixtral 8x22B & \cellcolor{orange!15.5} 0.29 & \cellcolor{orange!3.4} 0.29 & 0.54 & \cellcolor{cyan!0.5} 0.70 & \cellcolor{cyan!0.4} 0.71 & 0.06 \\
Mixtral 8x7B (it) & \cellcolor{cyan!0.3} 0.06 & \cellcolor{cyan!18.5} 0.19 & 0.69 & \cellcolor{cyan!22.2} 0.74 & 0.60 & 0.13 \\
Mixtral 8x7B & 0.20 & 0.25 & 0.56 & 0.70 & \cellcolor{cyan!10.2} 0.72 & 0.07 \\
Mistral 7B (it) & 0.07 & 0.20 & 0.67 & 0.65 & 0.65 & 0.20 \\
Mistral 7B & \cellcolor{orange!22.1} 0.30 & \cellcolor{orange!18.5} 0.30 & 0.50 & 0.70 & 0.70 & 0.05 \\
Yi 34B (it) & 0.22 & 0.24 & 0.57 & \cellcolor{orange!25.0} 0.31 & \cellcolor{cyan!0.4} 0.71 & 0.07 \\
Yi 34B & 0.09 & 0.20 & 0.67 & 0.64 & 0.64 & 0.15 \\
Gemma 7B (it) & 0.18 & 0.24 & 0.57 & 0.61 & 0.61 & 0.22 \\
Gemma 2B (it) & 0.24 & \cellcolor{orange!14.2} 0.29 & \cellcolor{orange!25.0} 0.42 & 0.42 & 0.70 & 0.17 \\
Gemma 7B & 0.18 & 0.26 & 0.48 & 0.70 & 0.70 & 0.11 \\
Gemma 2B & \cellcolor{orange!25.0} 0.30 & \cellcolor{orange!25.0} 0.30 & 0.50 & 0.70 & 0.70 & 0.02 \\
\midrule
LR & 0.03 & 0.19 & 0.70 & 0.72 & - & - \\
% GBM & 0.01 & 0.14 & 0.83 & 0.80 & - & - \\
XGBoost & 0.00 & 0.14 & 0.84 & 0.80 & - & - \\
\bottomrule
\end{tabular}


==> tables/numeric_prompting/acstraveltime.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{ECE $\downarrow$}} & \multirow{2}{*}{\textbf{\shortstack{Brier \\score}}} \multirow{2}{*}{$\downarrow$} & \multirow{2}{*}{\textbf{\shortstack{AUC}}} \multirow{2}{*}{$\uparrow$} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=0.5$}}} & \multirow{2}{*}{\textbf{\shortstack{Accuracy $\uparrow$\\ $\tau=t^\prime$}}} & \multirow{2}{*}{\textbf{\shortstack{Score $\sigma$ \\ st. dev.}}} \\ \\
\midrule
GPT 4o mini (it) & 0.15 & 0.27 & 0.58 & 0.57 & \cellcolor{orange!1.1} 0.51 & 0.22 \\
Llama 3 70B (it) & 0.12 & \cellcolor{cyan!22.5} 0.24 & \cellcolor{cyan!25.0} 0.64 & 0.53 & \cellcolor{cyan!22.8} 0.61 & 0.13 \\
Llama 3 70B & 0.08 & \cellcolor{cyan!12.4} 0.25 & 0.52 & 0.46 & 0.56 & 0.05 \\
Llama 3 8B (it) & 0.11 & \cellcolor{cyan!12.4} 0.25 & 0.56 & 0.56 & 0.52 & 0.06 \\
Llama 3 8B & 0.12 & 0.26 & \cellcolor{orange!25.0} 0.48 & \cellcolor{orange!25.0} 0.44 & 0.55 & 0.02 \\
Mixtral 8x22B (it) & 0.12 & \cellcolor{cyan!23.7} 0.24 & \cellcolor{cyan!23.5} 0.64 & \cellcolor{cyan!25.0} 0.59 & \cellcolor{cyan!25.0} 0.61 & 0.14 \\
Mixtral 8x22B & 0.30 & 0.34 & 0.57 & \cellcolor{cyan!2.4} 0.58 & 0.58 & 0.17 \\
Mixtral 8x7B (it) & 0.09 & \cellcolor{cyan!25.0} 0.24 & 0.61 & 0.57 & \cellcolor{orange!25.0} 0.50 & 0.11 \\
Mixtral 8x7B & 0.07 & \cellcolor{cyan!16.2} 0.25 & 0.57 & \cellcolor{cyan!2.4} 0.58 & 0.57 & 0.12 \\
Mistral 7B (it) & 0.11 & \cellcolor{cyan!11.2} 0.25 & 0.55 & 0.56 & \cellcolor{orange!25.0} 0.50 & 0.10 \\
Mistral 7B & \cellcolor{orange!25.0} 0.44 & \cellcolor{orange!25.0} 0.44 & 0.50 & 0.56 & 0.56 & 0.01 \\
Yi 34B (it) & \cellcolor{cyan!3.7} 0.06 & \cellcolor{cyan!11.2} 0.25 & 0.50 & \cellcolor{orange!25.0} 0.44 & 0.56 & 0.00 \\
Yi 34B & 0.14 & 0.27 & 0.53 & \cellcolor{orange!25.0} 0.44 & 0.57 & 0.07 \\
Gemma 7B (it) & 0.10 & \cellcolor{cyan!4.9} 0.26 & \cellcolor{orange!4.9} 0.49 & \cellcolor{orange!25.0} 0.44 & 0.56 & 0.01 \\
Gemma 2B (it) & 0.19 & 0.28 & 0.50 & 0.56 & 0.56 & 0.00 \\
Gemma 7B & \cellcolor{cyan!25.0} 0.03 & \cellcolor{cyan!13.7} 0.25 & 0.52 & 0.55 & 0.54 & 0.07 \\
Gemma 2B & \cellcolor{orange!25.0} 0.44 & \cellcolor{orange!25.0} 0.44 & 0.50 & 0.56 & 0.56 & 0.00 \\
\midrule
LR & 0.04 & 0.24 & 0.58 & 0.56 & - & - \\
% GBM & 0.02 & 0.20 & 0.75 & 0.69 & - & - \\
XGBoost & 0.02 & 0.19 & 0.77 & 0.70 & - & - \\
\bottomrule
\end{tabular}

